Safe Linear-Quadratic Dual Control with Almost Sure Performance Guarantee

This paper considers the linear-quadratic dual control problem where the system parameters need to be identified and the control objective needs to be optimized in the meantime. Contrary to existing works on data-driven linear-quadratic regulation, which typically provide error or regret bounds within a certain probability, we propose an online algorithm that guarantees the asymptotic optimality of the controller in the almost sure sense. Our dual control strategy consists of two parts: a switched controller with time-decaying exploration noise and Markov parameter inference based on the cross-correlation between the exploration noise and system output. Central to the almost sure performance guarantee is a safe switched control strategy that falls back to a known conservative but stable controller when the actual state deviates significantly from the target state. We prove that this switching strategy rules out any potential destabilizing controllers from being applied, while the performance gap between our switching strategy and the optimal linear state feedback is exponentially small. Under our dual control scheme, the parameter inference error scales as $O(T^{-1/4+\epsilon})$, while the suboptimality gap of control performance scales as $O(T^{-1/2+\epsilon})$, where $T$ is the number of time steps, and $\epsilon$ is an arbitrarily small positive number. Simulation results on an industrial process example are provided to illustrate the effectiveness of our proposed strategy.

==> algo.tex <==
\section{An online algorithm for simultaneous identification and control}\label{sec:algorithm}

\subsection{An online algorithm}

The complete algorithm we propose for simultaneous identification and control is presented in Algorithm~\ref{alg:main}. The notations are described later in this subsection.

\renewcommand{\algorithmicrequire}{\textbf{Initialization:}}
\renewcommand{\algorithmicensure}{\textbf{Iteration:}}

\begin{algorithm}
	\caption{Online LQR with simultaneous identification and control}
	\begin{algorithmic}[1]
		\Require $k \gets 0$
		\Ensure
		\While{$k < n+p$}
		\State Observe the current state $x_k$
		\State $\ut_k \gets 0$
		\State Generate random variable $\zeta_k \sim \gaussian{0}{I_p}$
 		\State Apply control input $u_k \gets \ut_k + (k+1)^{-\beta} \zeta_k$
		\State $k \gets k + 1$
		\EndWhile
		
		\While{true}
		\State Observe the current state $x_k$
		\For{$ \tau = 0, 1, \ldots, n + p - 1 $}
		    \State $\displaystyle \begin{aligned}\Hhat_{k,\tau} \gets & \frac{1}{k - \tau}\sum_{i=\tau + 1}^k  (i-\tau)^\beta \\ & \left[x_i - \sum_{t = 0}^{\tau - 1} \Hhat_{k, t} \ut_{i-t-1}  \right] \zeta_{i-\tau-1}^\top\end{aligned}$
		\EndFor
% 		\State Realize $\Ahat_k, \Bhat_k$ from $\Hhat_{k,0}, \ldots, \Hhat_{k,\min(n,k) - 1}$
% 		\State Restore $\Ahat_k, \Bhat_k$ from $\Hhat_{k,0}, \ldots, \Hhat_{k,2n-1}$ using Algorithm~\ref{alg:ho_kalman}
        \State Reconstruct $\Ahat_k, \Bhat_k$ from $\Hhat_{k,0}, \ldots, \Hhat_{k,n+p-1}$ using Algorithm~\ref{alg:dd_lsq}
		\State Compute $\Khat_k$ by replacing $A, B$ with $\Ahat_k, \Bhat_k$ in~\eqref{eq:dare},\eqref{eq:K}
		\State $\uhat_k \gets \Khat_k x_k$
		\State $\ut_k \gets \proj{\uhat_k}{C\log(k+1)}$, where $\proj{v}{M}$ is defined as the projection of vector $v$ onto the Euclidean ball $\{x: \norm{x} \leq M\}$
		\State Generate random variable $\zeta_k \sim \gaussian{0}{I_p}$
		\State Apply control input $u_k \gets \ut_k + (k+1)^{-\beta} \zeta_k$
		\State $k \gets k + 1$
		
		\EndWhile
	\end{algorithmic}
	\label{alg:main}
\end{algorithm}

\subsubsection{Generation of control input}

Let us design the control input $u_k$, which can be considered an approximation of the optimal control input based on the knowledge up to step $k$. We use purely random input for the first $n + p$ steps since we have not gathered sufficient information about the system. Starting from time step $n + p$, we choose the input as
\begin{equation}
    u_k = \ut_k + k^{-\beta} \zeta_k = \proj{\uhat_k}{C\log(k+1)} + k^{-\beta} \zeta_k,
    \label{eq:input}
\end{equation}
where $0 < \beta < 1/2, C > 0$ are constants, $\zeta_k$'s are i.i.d. Gaussian random vectors with identity covariance, $\uhat_k = \Khat_k x_k$ is the optimal control input for the currently estimated system $\left( \Ahat_k, \Bhat_k \right)$, and $\ut_k$ is the projection of $\uhat_k$ onto the Euclidean ball $\{x: \norm{x} \leq C\log(k+1)\}$.

\begin{remark}
Notice that the second term $k^{-\beta} \zeta_k$ on the RHS of~\eqref{eq:input} is crucial for parameter identification. The reason is that $\ut_k$ is ``greedy'' in the sense that its direction is optimal based on knowledge up to step $k$, and hence it in general does not provide persistent excitation in every direction, which is necessary to identify all the system parameters. Conceptually, the $k^{-\beta} \zeta_k$ can be interpreted as an ``exploration'' term, as its randomness provides excitation required to the system for us to infer the parameters. In contrast, the $\ut_k$ term can be interpreted as the ``exploitation'' term, as it depends deterministically on our current knowledge of the system parameters.
\end{remark}

\begin{remark}
Notice that we use $\ut_k$ instead of $\uhat_k$ as the ``exploitation'' term on the RHS of~\eqref{eq:input}. Actually, $\ut_k$ is a ``saturated'' version of $\uhat_k$, with the maximum allowed Euclidean norm $C\log(k+1)$ growing at a logarithmic rate as the time $k$ increases. The saturation mechanism averts excessive inputs caused by inaccurate parameter estimates in the initial stage, which is essential to guarantee the convergence of our inference algorithm. Meanwhile, the logarithmic growth of the saturation threshold is sufficient to ensure that the saturation has practically no effect on the asymptotic control performance.
\end{remark}

\subsubsection{Inference of system parameters}

The Markov parameters of the system described in~\eqref{eq:dynamics} are defined as
\begin{equation}
    H_\tau \triangleq A^\tau B, \quad \tau = 0,1,\ldots.
    \label{eq:markov}
\end{equation}
The Markov parameter sequence $\left\{ H_\tau \right\}_{\tau=0}^\infty$ can be interpreted as the impulse response of the system. It shall be noted that finite terms of the Markov parameter sequence would be sufficient to characterize the system, since higher-order Markov parameters can be represented as the linear combination of lower-order Markov parameters using the characteristic polynomial of $A$ in combination with Cayley-Hamilton theorem. Therefore, the purpose of our inference algorithm is to estimate $\left\{ H_\tau \right\}_{\tau=0}^{n+p-1}$, the first $n+p$ terms of the impulse response. In what follows, we denote our estimate of $H_\tau$ at step $k$ by $\Hhat_{k,\tau}$.

To explain the inference algorithm, we can cast the system~\eqref{eq:dynamics} into a static form by writing $x_k$ as
\begin{align}
     x_k &= A^k x_0 + \sum_{t=0}^{k-1} A^t B u_{k-t - 1} + \sum_{t=0}^{k-1}A^t w_{k-t-1}
    \label{eq:static}\\
     & \begin{aligned}= A^k x_0 + \sum_{t=0}^{k-1} H_t \left[ \ut_{k-t - 1} + ({k-t})^{-\beta} \zeta_{k-t - 1} \right] + \\ \sum_{t=0}^{k-1}A^t w_{k-t-1}, \end{aligned}
    \label{eq:static_substituted}
\end{align}
where the second equality follows by substituting~\eqref{eq:input} and \eqref{eq:markov} into~\eqref{eq:static}. Now in order to estimate $H_\tau$, post-multiply both sides of~\eqref{eq:static_substituted} with $\zeta_{k - \tau - 1}^\top$ and rearrange the terms, and we get
\begin{equation}
\begin{aligned}
    x_k \zeta_{k - \tau - 1}^\top = \left( \sum_{t=0}^{k-1}A^t w_{k-t-1} +A^k x_0 \right) \zeta_{k - \tau - 1}^\top + \\ \sum_{t=0}^{k-1} ({k-t})^{-\beta} H_t\zeta_{k-t - 1} \zeta_{k - \tau - 1}^\top + \\ \sum_{t=0}^{k-1} H_t \ut_{k-t - 1} \zeta_{k - \tau - 1}^\top.
\end{aligned}
\label{eq:intuition}
\end{equation}
Notice that $x_0, \zeta_0, \zeta_1, \ldots, \zeta_k, w_0, w_1, \ldots, w_k$ are zero mean independent Gaussian random vectors. Roughly speaking, viewed from the sense of expectation, the first term on the RHS of~\eqref{eq:intuition} can be ignored due to the statistical independence between $\zeta_{k-\tau-1}$ and the initial state $x_0$ and process noise $w$'s. Similarly, the summation in the second term on the RHS of~\eqref{eq:intuition} can be reduced to a single item where $t=\tau$ due to the statistical independence between $\zeta$'s at different steps. Finally, in the summation in the third term on the RHS of~\eqref{eq:intuition}, the items where $t=\tau, \tau+1, \ldots, k-1$ can be ignored following a similar argument. However, the items where $t=0, 1, \ldots, \tau - 1$ cannot be ignored because later $\ut$'s would depend on earlier $\zeta$'s.

Motivated by the above intuitions, we can recursively define
\begin{equation}
    \Hhat_{k,\tau} \triangleq \frac{1}{k - \tau}\sum_{i=\tau + 1}^k  (i-\tau)^\beta \left[x_i - \sum_{t = 0}^{\tau - 1} \Hhat_{k, t} \ut_{i-t-1}  \right] \zeta_{i-\tau-1}^\top,
    \label{eq:Hktau}
\end{equation}
where $\tau = 0,1,\ldots, k-1$. The convergence of the estimated Markov parameters $\Hhat_{k,\tau}$ to the true Markov parameters $H_{\tau}$ can be established through a convergence theorem of matrix-valued martingales, and a rigorous proof is given in the next subsection.

\begin{remark}
As a computational remark, it should be noted that~\eqref{eq:markov} can be decomposed to enable efficient recursive computation. To see this, we can rearrange~\eqref{eq:markov} as
\begin{equation*}
    \begin{aligned}
    \Hhat_{k,\tau} &= \frac{1}{k - \tau}\sum_{i=\tau + 1}^k  (i-\tau)^\beta x_i\zeta_{i-\tau-1}^\top  \\
    &- \sum_{t=0}^{\tau - 1} \Hhat_{k,t} \left[ \frac{1}{k - \tau} \sum_{i=\tau + 1}^k  (i-\tau)^\beta \ut_{i-t-1} \zeta_{i-\tau-1}^\top \right],
    \end{aligned}
    % \label{eq:cum_avg}
\end{equation*}
the weighted sum of $\tau + 1$ cumulative averages, each of which can be updated with a constant amount of computation in each step. Therefore, the time complexity of each iteration and the total memory consumption are constant. 
\end{remark}

\subsubsection{Approximate control law based on estimated parameters}

Given the estimated finite Markov parameter sequence $\left\{ \Hhat_{k,\tau} \right\}_{\tau=0}^{n+p-1}$, we can accordingly obtain an estimate $\Ahat_k, \Bhat_k$ of the true system parameters $A, B$, such that the system described by $\left(\Ahat_k, \Bhat_k\right)$ has an impulse response as similar to $\left\{ \Hhat_{k,\tau} \right\}_{\tau=0}^{n+p-1}$ as possible. To this end, we can generate simulated state and input trajectories from $\left\{ \Hhat_{k,\tau} \right\}_{\tau=0}^{n+p-1}$, and estimate $\Ahat_k, \Bhat_k$ using a least-squares approach. The above-described procedure is detailed in Algorithm~\ref{alg:dd_lsq}. Finally, an approximate feedback gain $\Khat_k$ can be easily derived from $\Ahat_k, \Bhat_k$ by solving the discrete-time algebraic Riccati equation.

% The idea is based on the celebrated Ho-Kalman algorithm~\cite{Ho_Kalman} for the minimal state space realization problem. When $(A,B)$ is controllable, the order of the minimal realization is equal to the order of $A$. Furthermore, in our case, the state can directly be measured, which can be seen as the observation matrix being the identity matrix. By performing a coordinate transform, we can obtain a unique minimal realization with identity observation matrix. The above described procedure is detailed in Algorithm~\ref{alg:ho_kalman}.

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

% \begin{algorithm}
% 	\caption{Restoring system parameters from Markov parameters}
% 	\begin{algorithmic}[1]
% 		\Require Markov parameter estimate sequence $\Hhat_0, \Hhat_1, \ldots, \Hhat_{2n-1}$
% 		\Ensure System parameter estimate $\Ahat, \Bhat$
% 		\State $\Bhat \gets \Hhat_0$
% 		\State Form block Hankel matrices
% 		\begin{equation*}
% 		    \Hankel_{n,n} = \begin{bmatrix}
%                 \Hhat_0 & \Hhat_1 & \cdots & \Hhat_{n-1} \\
%                 \Hhat_1 & \Hhat_2 & \cdots & \Hhat_n \\
%                 \vdots & \vdots & \ddots & \vdots \\
%                 \Hhat_{n-1} & \Hhat_n & \cdots & \Hhat_{2n-2}
%             \end{bmatrix},
% 		    \bar{\Hankel}_{n,n} = \begin{bmatrix}
%                 \Hhat_1 & \Hhat_2 & \cdots & \Hhat_{n} \\
%                 \Hhat_2 & \Hhat_3 & \cdots & \Hhat_{n+1} \\
%                 \vdots & \vdots & \ddots & \vdots \\
%                 \Hhat_{n} & \Hhat_{n+1} & \cdots & \Hhat_{2n-1}
%             \end{bmatrix}
% 		\end{equation*}
		
% 		\State $U_n, \Sigma_n, V_n \gets \mathrm{SVD} \left( \Hankel_{n,n}  \right)$, where reduced SVD is used, i.e., $U_n\in \R{n^2 \times n}, \Sigma_n \in \R{n \times n}, V_n \in \R{np\times n}$
% 		\State $H_o \gets U_n\Sigma_n^{1/2}, H_c \gets \Sigma_n^{1/2} V_n^\top$
% 		\State Obtain minimal realization $\Ahat'\gets H_o^\dag \bar{\Hankel}_{n,n} H_c^\dag, \Bhat' \gets H_c(:, 1:p), \Chat' \gets H_o(1:n, :)$, where $\left( \cdot \right)^\dag$ stands for the pseudo-inverse, $H_c(:, 1:p)$ stands for the first $p$ columns of $H_c$, and $H_o(1:n, :)$ stands for the first $n$ rows of $H_o$
% 		\State Perform coordinate transform to obtain $\Ahat \gets \Chat' \Ahat' \left( \Chat' \right)^{-1}$
% 	\end{algorithmic}
% 	\label{alg:ho_kalman}
% \end{algorithm}

\begin{algorithm}
    \caption{Restoring system matrices from Markov parameters}
    \begin{algorithmic}[1]
        \Require Markov parameter estimate sequence $\Hhat_0, \Hhat_1, \ldots, \Hhat_{n+p-1}$, number of simulated trajectories $N$
        \Ensure System matrices estimate $\Ahat, \Bhat$
        \State Construct block Toeplitz matrix
		\begin{equation*}
		    \Toep \gets \begin{bmatrix}
                0 & 0 & 0 & \cdots & 0 \\
                \Hhat_0 & 0 & 0 & \cdots & 0 \\
                \Hhat_1 & \Hhat_0 & 0 & \cdots & 0 \\
                \vdots & \vdots & \vdots & \ddots & \vdots \\
                \Hhat_{n+p-1} & \Hhat_{n+p-2} & \Hhat_{n+p - 3} & \cdots & 0
            \end{bmatrix}
		\end{equation*}
		\State Choose $N$ independent random input trajectories, each $(n+p)$-long, denoted by
		\begin{equation*}
		    \ustep{i} \gets \begin{bmatrix}
                u_i^{(1)} & u_i^{(2)} & \cdots & u_i^{(N)} \end{bmatrix}, \quad i=0,1,\ldots,n+p-1.
		\end{equation*}
        \State Stack the inputs vertically and compute states:
        \begin{align*}
            &\Uvert \gets \begin{bmatrix}
            \ustep{0} \\ \ustep{1} \\ \vdots \\ \ustep{n+p-1}
            \end{bmatrix},
            \begin{bmatrix}
            \xstep{1} \\ \xstep{2} \\ \vdots \\ \xstep{n+p}
            \end{bmatrix} =: \Xvert \gets \Toep \Uvert
        \end{align*}
        \State Stack the inputs and states horizontally to form the following matrices:
        \begin{align*}
            &\Uhori \gets \begin{bmatrix}
            \ustep{0} & \ustep{1} & \cdots & \ustep{n+p-1}
            \end{bmatrix}, \\
            &\Xhorione \gets \begin{bmatrix}
            \xstep{1} & \xstep{2} & \cdots & \xstep{n+p}
            \end{bmatrix}, \\
            &\Xhorizero \gets \begin{bmatrix}
            \mathbf{0}_{n\times N} & \xstep{1} & \cdots & \xstep{n+p-1}
            \end{bmatrix}
        \end{align*}
        \State Compute estimate
        \begin{align*}
            \begin{bmatrix} \Bhat & \Ahat \end{bmatrix} \gets \Xhorione \begin{bmatrix} \Uhori \\ \Xhorizero \end{bmatrix}^\dag,
        \end{align*}

    \end{algorithmic}
    \label{alg:dd_lsq}
\end{algorithm}

It can be shown the procedure described in Algorithm~\ref{alg:dd_lsq} restores the actual system matrices as long as the Markov parameter estimates are accurate.

\begin{lemma} \cite{data_driven_control, Willems}
Assuming $(A, B)$ is controllable, when $\Hhat_\tau = H_\tau = A^\tau B$ for all $\tau = 0,1,\ldots, n+p-1$, and the matrix $\begin{bmatrix} \Uhori \\ \Xhorizero \end{bmatrix}$ defined in Algorithm~\ref{alg:dd_lsq} has full row rank, then the result of Algorithm~\ref{alg:dd_lsq} satisfies $\Ahat = A, \Bhat = B$.
\label{lemma:ddlsq_consistency}
\end{lemma}

\begin{remark}
Lemma~\ref{lemma:ddlsq_consistency} guarantees the consistency of our approximate control law, i.e., accurate Markov parameter estimates would generate an accurate control law, which is crucial for the asymptotic optimality of the controller. The rank condition in Lemma~\ref{lemma:ddlsq_consistency} guarantees that the inputs provide sufficient excitation to reconstruct system matrices from impulse responses, and is easily satisfied by randomly generated inputs. For the ease of analysis, it is also legitimate to use fixed, rather than random $\ustep{i}$'s for each time step $k$ of the outer loop of Algorithm~\ref{alg:main}, as long as the rank condition is satisfied.
\end{remark}

==> algo_prop_long.tex <==
\subsection{Convergence analysis}

The following two theorems respectively establish the convergence of the parameter estimates and the performance of the control policy.

\begin{theorem}
Assuming $A$ is strictly stable. If $0 < \beta < 1/2$, then for any $\epsilon > 0$, the following limit holds almost surely:
\begin{equation}
    \lim_{k\to\infty} \frac{\Hhat_{k,\tau} - H_\tau}{k^{-\gamma + \epsilon}} = 0,
    \label{eq:converge_H}
\end{equation}
where $\gamma = 1/2 - \beta > 0$, for $\tau = 0,1, \ldots, n-1$. In particular, $\Hhat_{k,\tau}$ almost surely converges to $H_\tau$ for $\tau = 0,1, \ldots, n-1$.
\label{thm:converge_H}
\end{theorem}

% Before characterizing the convergence of control performance, it is worth noticing that our saturation scheme is nonlinear, posing significant difficulty to the analysis of the closed-loop system. Therefore, we resort to the technique of stochastic linearization, which approximates the nonlinear saturation unit as quasilinear unit whose gain is a function of the variance of its input signal. The quality of this approximation has been numerically validated in previous research; for more details about stochastic linearization, please refer to~\cite{stochastic_linearization,slqr}.

\begin{theorem}
Assuming $A$ is strictly stable, and $0 < \beta < 1/2$. Let $\pi_k$ be the control policy used at step $k$, i.e., $\pi_k(x) = \proj{\Khat_k x}{C\log(k+1)} + k^{-\beta}\zeta, \zeta \sim \gaussian{0}{I_p}$,
% Let $J^*$ be the optimal cost defined in~\eqref{eq:J_opt} and $\hat{J}^{\pi_k}$ be the cost of the stochastically linearized closed-loop system under $\pi_k$, then for any $\epsilon > 0$, the following limit holds almost surely:
then with $J^{\pi_k}$ and $J^*$ defined in~\eqref{eq:J_pi}, \eqref{eq:J_opt} respectively, for any $\epsilon > 0$, the following limit holds almost surely:
\begin{equation}
    \lim_{k\to\infty} \frac{J^{\pi_k} - J^*}{k^{-\min(\beta,2\gamma) + \epsilon}} = 0,
    \label{eq:converge_J}
\end{equation}
where $\gamma = 1/2 - \beta > 0$. In particular, $J^{\pi_k}$ almost surely converges to $J^*$.
\label{thm:converge_J}
\end{theorem}

\begin{remark}
It is worth noticing that~\eqref{eq:converge_H} implies that the Markov parameter estimates converge at the order $\O\left( k^{-\gamma + \epsilon} \right)$. Hence, the convergence rate $\gamma$ is maximized when $\beta \to 0^+$.
However, the exploration term $k^{-\beta}$ does not decay in this case, and the control performance $J^{\pi_k}$ will not converge to the optimal performance $J^*$. To achieve the fastest convergence of $J^{\pi_k}$, we need to choose the decay rate of the exploration term to be $\beta = 1/3$, which maximizes $\min(\beta, 2\gamma) = \min(\beta, 1-2\beta)$.
\end{remark}

The proof of Theorem~\ref{thm:converge_H} is based on a convergence result for matrix-valued martingales. To simplify notations, for a random variable (vector, or matrix) sequence $\left\{ x_k \right\}$, we denote that $x_k \sim \C(\alpha)$ if for all $\epsilon > 0$, we have $x_k \sim \O\left( k^{\alpha + \epsilon} \right)$, i.e.,
$
    \lim _{k \rightarrow \infty} \left\|x_{k}\right\| / {k^{\alpha+\epsilon}} \stackrel{a . s .}{=} 0.
$
\footnote{Notice that $x_k \sim \O\left( k^\alpha \right)$ implies $x_k \sim \C(\alpha)$, but the reverse is not true, e.g., $k^\alpha \log k \sim \C(\alpha)$ but not $k^\alpha \log k \nsim \O\left( k^\alpha \right)$.}
The following lemma establishes some basic properties of $\C(\alpha)$ functions:

\begin{lemma} \cite[Lemma 3]{watermark}
Assume $x_k, y_k$ are random variable (vector, or matrix) sequences with proper dimensions, then the following properties hold: \begin{enumerate}
    \item $x_k \sim \C(\alpha)$ if and only if $\norm{x_k} \sim \C(\alpha)$.
    \item If $x_k \sim \C(\alpha), y_k \sim \C(\beta)$, then $x_k + y_k \sim \C\left( \max(\alpha, \beta) \right)$.
    \item If $x_k \sim \C(\alpha), y_k \sim \C(\beta)$, then $x_k y_k \sim \C(\alpha + \beta)$.
    \item If $x_{k+1} = A x_k + r_k$, with $A$ being strictly stable and $r_k \sim \C(\alpha)$, then $x_k \sim \C(\alpha)$.
    \item If $x_k$ are i.i.d. Gaussian random variables (vectors), then $x_k \sim \C(0)$.
    \item If $f$ is a function differentiable at 0 and $x_k \sim C(\alpha), \alpha < 0$, then $f\left( x_k \right) - f(0) \sim C(\alpha)$.
\end{enumerate}
\label{lemma:function_class}
\end{lemma}

% \begin{proof}
% See~\cite[Lemma 3]{watermark}. 
% \end{proof}

Let $\left\{ \F_k \right\}$ be a filtration of $\sigma$-algebras and $\left\{ M_k \right\}$ be a matrix-valued stochastic process adapted to $\left\{ \F_k \right\}$, we call $\left\{ M_k \right\}$ a matrix-valued martingale (with respect to the filtration $\left\{ \F_k \right\}$) if the $\E\left( M_{k+1} \mid \F_k \right) = M_k$ holds for all $k$.
We shall assume throughout the paper that $\left\{ \F_k \right\}$ is the $\sigma$-algebra generated by the random variables $\left\{ x_0, w_0, \ldots, w_k, \zeta_0, \ldots, \zeta_k \right\}$. Now we can state a strong law for matrix-valued martingales:

\begin{lemma} \cite[Lemma 4]{watermark}
If $M_k = \Phi_0 + \Phi_1 + \cdots + \Phi_k$ is a matrix-valued martingale such that
\begin{equation*}
    \E \norm{\Phi_k}^2 \sim \C(\beta),
\end{equation*}
where $0\leq \beta < 1$, then $M_k / k$ converges to 0 almost surely. Furthermore,
\begin{equation*}
\frac{M_{k}}{k} \sim \mathcal{C}\left(\frac{\beta-1}{2}\right).
\end{equation*}
\label{lemma:martingale}
\end{lemma}

% \begin{proof}
% See~\cite[Lemma 4]{watermark}. 
% \end{proof}

The next two lemmas bound the growth of the fourth-order moment of the norm of the state vector under our input saturation scheme.

\begin{lemma}
Assume $\left\{ x_k : k \geq 1 \right\}$ is a positive scalar sequence satisfying $x_{k+1} = ax_k + b\sqrt{x_k}\log(k+1) + c\left( \log(k+1) \right)^2$, where $0 < a < 1, b>0,c>0,\alpha > 0$, then
\begin{equation*}
    x_k \leq M^2 \left( \log(k+1) \right)^2
\end{equation*}
for every $k$, where $M = \max\left( \frac{\sqrt{x_1}}{\log(2)}, \frac{b + \sqrt{b^2 + 4c(1-a)}}{2(1-a)} \right)$.
\label{lemma:Ex2_recursion}
\end{lemma}

\begin{proof}
The result follows trivially from induction on $k$.
\end{proof}


\begin{lemma}
With the system described in~\eqref{eq:dynamics} and control input determined by Algorithm~\ref{alg:main}, assuming $A$ is strictly stable, 
then as $k\to\infty$,
\begin{align}
&\E\norm{x_k}^2 \sim \O\left( \left( \log k \right)^2 \right), \label{eq:Ex2}\\
&\E\norm{x_k}^4 \sim \O\left( \left( \log k \right)^4 \right). \label{eq:Ex4}
\end{align}
\label{lemma:Ex4}
\end{lemma}

\renewcommand*{\proofname}{Proof}

\begin{proof}
Suppose $A$ is strictly stable but not contractive, i.e., $\rho(A) < 1, \norm{A} \geq 1$. Let $P$ be the unique positive definite solution to the Lyapunov equation $A^\top PA - P + I = 0$ and perform a coordinate transformation of the system using $T = P^{-1/2}$. It can be shown $\tilde{A} = T^{-1} A T$ satisfies $\norm{\tilde{A}} < 1$, and the conclusion is satisfied by the original system when satisfied by the transformed system. Therefore, we may assume $\norm{A} < 1$ for the rest of the proof.

When $\norm{A} < 1$,
From~\eqref{eq:dynamics} we have
\begin{align}
    \norm{x_{k+1}}^2 &= x_k^\top A^\top A x_k + 2 \left(Bu_k + w_k \right)^\top A x_k + u_k^\top B^\top B u_k + 2w_k^\top B^\top u_k + \norm{w_k}^2.
    \label{eq:x2}
\end{align}
Since $w_k \sim \gaussian{0}{I_n}$ and $\norm{u_k}\leq C\log(k+1)$, and $w_k$ is independent from $x_k$ and $u_k$, there is
\begin{align*}
    \E\norm{x_{k+1}}^2 &\leq \norm{A}^2 \E\norm{x_k}^2 + 2C\norm{B^\top A}\E\norm{x_k}\log(k+1) + 2C^2\norm{B}^2 \left( \log(k+1) \right)^2 + n  \\
    & \leq \norm{A}^2 \E\norm{x_k}^2 + b\sqrt{\E\norm{x_k}^2} \log(k+1) + c\left( \log(k+1) \right)^2 ,
\end{align*}
with properly chosen constants $b>0, c>0$ for sufficiently large $k$. Since $0 < \norm{A} < 1$, \eqref{eq:Ex2} follows from Lemma~\ref{lemma:Ex2_recursion}.

Furthermore, from~\eqref{eq:x2} and $\norm{u_k}\leq C\log(k+1)$ we have
\begin{align*}
    \norm{x_{k+1}}^2 &\leq \norm{A}^2 \norm{x_k}^2 + 2\norm{A^\top}\left( C\norm{B}\log(k+1) + \norm{w_k} \right) \norm{x_k} + C^2\norm{B}^2 \left( \log(k+1) \right)^2 + \\&\mkern108mu 2C\norm{B}\log(k+1) + \norm{w_k}^2, \\
    &\leq \norm{A}^2 \norm{x_k}^2 + \left( c_1+c_2 \norm{w_k} \right)\norm{x_k}\log(k+1) + c_3 \left( \log(k+1) \right)^2 + \norm{w_k}^2,
\end{align*}
where the last inequality holds for sufficiently large $k$ with properly chosen constants $c_1, c_2, c_3 > 0$. Hence,
\begin{equation}
\begin{aligned}
    \norm{x_{k+1}}^4 \leq & \norm{A}^4 \norm{x_k}^4 + 2\norm{A}^2\left( c_1+c_2 \norm{w_k} \right)\norm{x_k}^3 + \\
    & \left[ 2\norm{A}^2c_3 \left( \log(k+1) \right)^2 +  2\norm{A}^2\norm{w_k}^2 + 3\left( c_1 + c_2 \norm{w_k} \right)^2 \right] \norm{x_k}^2 + \\
    & 3c_3\left( \log(k+1) \right)^4 + 3\norm{w_k}^4,
\end{aligned}
\label{eq:x4}
\end{equation}
where we used the fact $(x+y+z+w)^2 \leq x^2 + 2x(y+z+w) + 3(y^2+z^2+w^2)$. Since $w_k \sim \gaussian{0}{W}$, there is $\E\norm{w_k}^2 = \Tr(W), \E\norm{w_k}^4 = \Tr(W)\left(\Tr(W)+2\right), \E\norm{w_k} \leq \sqrt{\E\norm{w_k}^2} = \sqrt{\Tr(W)}$. Taking expectation over both sides of~\eqref{eq:x4}, noting the fact that $x_k$ and $w_k$ are independent, and abbreviating the constants, we get
\begin{align*}
    \E\norm{x_{k+1}}^4 \leq \norm{A}^4 \E\norm{x_k}^4 + c_4 \E\norm{x_k}^3 + c_5 \left( \log(k+1) \right)^2 \E\norm{x_k}^2 + c_6 \left( \log(k+1) \right)^4 + c_7 \E \norm{x_k}^2,
\end{align*}
where $c_3, c_4, c_5, c_6, c_7 > 0$. By Cauchy-Swartz inequality,
\begin{align*}
    \E\norm{x_k}^3 \leq \sqrt{\E\norm{x_k}^4 \E\norm{x_k}^2},
\end{align*}
and in view of~\eqref{eq:Ex2}, we have
\begin{align*}
    \E\norm{x_{k+1}}^4 \leq \norm{A}^4 \E\norm{x_k}^4 + c_8 \left( \log(k+1) \right) \sqrt{\E\norm{x_k}^4} + c_9 \left( \log(k+1) \right)^4,
\end{align*}
where $c_7, c_8, c_9 > 0$. By applying Lemma~\ref{lemma:Ex2_recursion} with $2\alpha$ in place of $\alpha$, we reach~\eqref{eq:Ex4}.
\end{proof}


% \begin{proof}

% Suppose $A$ is strictly stable but not contractive, i.e., $\rho(A) < 1, \norm{A} \geq 1$. Let $P$ be the unique positive definite solution to the Lyapunov equation $A^\top PA - P + I = 0$ and perform a coordinate transform of the system using $T = P^{-1/2}$. It can be shown $\tilde{A} = T^{-1} A T$ satisfies $\norm{\tilde{A}} < 1$, and the conclusion of this lemma is satisfied by the original system as long as it is satisfied by the transformed system. Therefore, we assume $\norm{A} < 1$ for the rest of the proof.

% From~\eqref{eq:dynamics} we have
% \begin{align}
%     \norm{x_{k+1}}^2 &= x_k^\top A^\top A x_k + 2 \left(Bu_k + w_k \right)^\top A x_k + u_k^\top B^\top B u_k + 2w_k^\top B^\top u_k + \norm{w_k}^2.
%     \label{eq:x2}
% \end{align}
% Since $w_k \sim \gaussian{0}{I_n}$ and $\norm{u_k}\leq C\log(k+1)$, and $w_k$ is independent from $x_k$ and $u_k$, there is
% \begin{align*}
%     \E\norm{x_{k+1}}^2 &\leq \norm{A}^2 \E\norm{x_k}^2 + 2C\norm{B^\top A}\E\norm{x_k}\log(k+1) + 2C^2\norm{B}^2 \left( \log(k+1) \right)^2 + n  \\
%     & \leq \norm{A}^2 \E\norm{x_k}^2 + b\sqrt{\E\norm{x_k}^2} \log(k+1) + c\left( \log(k+1) \right)^2 ,
% \end{align*}
% with properly chosen constants $b>0, c>0$ for sufficiently large $k$. Since $0 < \norm{A} < 1$, \eqref{eq:Ex2} follows from Lemma~\ref{lemma:Ex2_recursion}.

% Furthermore, from~\eqref{eq:x2} and $\norm{u_k}\leq C\log(k+1)$ we have
% \begin{align*}
%     \norm{x_{k+1}}^2 &\leq \norm{A}^2 \norm{x_k}^2 + 2\norm{A^\top}\left( C\norm{B}\log(k+1) + \norm{w_k} \right) \norm{x_k} + C^2\norm{B}^2 \left( \log(k+1) \right)^2 + \\&\mkern108mu 2C\norm{B}\log(k+1) + \norm{w_k}^2, \\
%     &\leq \norm{A}^2 \norm{x_k}^2 + \left( c_1+c_2 \norm{w_k} \right)\norm{x_k}\log(k+1) + c_3 \left( \log(k+1) \right)^2 + \norm{w_k}^2,
% \end{align*}
% where the last inequality holds for sufficiently large $k$ with properly chosen constants $c_1, c_2, c_3 > 0$. Hence,
% \begin{equation}
% \begin{aligned}
%     \norm{x_{k+1}}^4 \leq & \norm{A}^4 \norm{x_k}^4 + 2\norm{A}^2\left( c_1+c_2 \norm{w_k} \right)\norm{x_k}^3 + \\
%     & \left[ 2\norm{A}^2c_3 \left( \log(k+1) \right)^2 +  2\norm{A}^2\norm{w_k}^2 + 3\left( c_1 + c_2 \norm{w_k} \right)^2 \right] \norm{x_k}^2 + \\
%     & 3c_3\left( \log(k+1) \right)^4 + 3\norm{w_k}^4,
% \end{aligned}
% \label{eq:x4}
% \end{equation}
% where we used the fact $(x+y+z+w)^2 \leq x^2 + 2x(y+z+w) + 3(y^2+z^2+w^2)$. Since $w_k \sim \gaussian{0}{W}$, there is $\E\norm{w_k}^2 = \Tr(W), \E\norm{w_k}^4 = \Tr(W)\left(\Tr(W)+2\right), \E\norm{w_k} \leq \sqrt{\E\norm{w_k}^2} = \sqrt{\Tr(W)}$. Taking expectation over both sides of~\eqref{eq:x4}, noting the fact that $x_k$ and $w_k$ are independent, and abbreviating the constants, we get
% \begin{align}
%     \E\norm{x_{k+1}}^4 \leq \norm{A}^4 \E\norm{x_k}^4 + c_4 \E\norm{x_k}^3 + c_5 \left( \log(k+1) \right)^2 \E\norm{x_k}^2 + c_6 \left( \log(k+1) \right)^4 + c_7 \E \norm{x_k}^2,
% \end{align}
% where $c_3, c_4, c_5, c_6, c_7 > 0$. By Cauchy-Swartz inequality,
% \begin{align}
%     \E\norm{x_k}^3 \leq \sqrt{\E\norm{x_k}^4 \E\norm{x_k}^2},
% \end{align}
% and in view of~\eqref{eq:Ex2}, we have
% \begin{align}
%     \E\norm{x_{k+1}}^4 \leq \norm{A}^4 \E\norm{x_k}^4 + c_8 \left( \log(k+1) \right) \sqrt{\E\norm{x_k}^4} + c_9 \left( \log(k+1) \right)^4,
% \end{align}
% where $c_7, c_8, c_9 > 0$. By applying Lemma~\ref{lemma:Ex2_recursion} with $2\alpha$ in place of $\alpha$, we reach~\eqref{eq:Ex4}.
% \end{proof}


% \begin{lemma}
% Assuming $A$ is strictly stable. If $0 < \beta < \frac{1}{2}$ and $0 < \alpha < \frac{1}{2} - \beta$, there is
% \begin{equation*}
%     \Hhat_{k, \tau} - H_\tau \sim \C\left(\alpha + \beta - \frac{1}{2}\right),
% \end{equation*}
% for $\tau = 0,1,\ldots, n-1$.
% \end{lemma}

Now we are ready to prove Theorem~\ref{thm:converge_H}.

\renewcommand*{\proofname}{Proof of Theorem~\ref{thm:converge_H}}
% \renewcommand*{\proofname}{Proof of Theorem~\ref{thm:converge_H}}

\begin{proof}

As a preliminary result, notice that for any time step $k$, the variables $x_0, \zeta_0, \zeta_1, \ldots, \zeta_k$, $w_0, w_1, \ldots, w_k, \ut_0, \ut_1, \ldots, \ut_{k+1}$ are measurable w.r.t. $\F_k$, which, together with the independence among $x_0, \zeta_0, \zeta_1, \ldots, \zeta_k, w_0, w_1, \ldots, w_k$, leads to the following relations:
\begin{align}
  & \E\left( \zeta_{k_1} \zeta_{k_2}^\top \mid \F_{k_2 - 1} \right) = 
  \begin{cases} 
    I & \text{if } k_1 = k_2 \\
    0 & \text{otherwise},
  \end{cases} 
  \label{eq:zeta_zeta}
  \\
  & \E\left( \ut_{k_1} \zeta_{k_2}^\top \mid \F_{k_2-1} \right) = \begin{cases}
  0 & \text{if } k_1 \leq k_2 \\
  \text{other values} & \text{otherwise},
  \end{cases}
  \label{eq:u_zeta}
  \\
  &\E\left( w_{k_1} \zeta_{k_2}^\top \mid \F_{k_2-1} \right) = 0, 
  \label{eq:w_zeta} \\
  & \E\left( x_0 \zeta_{k_2}^\top \mid \F_{k_2-1} \right) = 0,
  \label{eq:x0_zeta}
\end{align}
for any two time steps $k_1 \geq 0$ and $k_2 \geq 1$.

Now let us prove the conclusion using induction on $\tau$.

First consider the case $\tau = 0$: we have
\begin{equation}
\Hhat_{k,0} - H_0 = \frac1k \sum_{i=1}^k \left[(i+1)^\beta x_i \zeta_{i-1}^\top - H_0 \right]= \frac1k \sum_{i=0}^{k-1} \left( (i+2)^\beta x_{i+1} \zeta_{i}^\top - H_0\right).
\label{eq:H0}
\end{equation}
Let $\Phi_k = (k+1)^\beta x_{k+1} \zeta_{k}^\top - H_0$. By substituting~\eqref{eq:static_substituted} and~\eqref{eq:zeta_zeta} to \eqref{eq:x0_zeta} into~\eqref{eq:H0} it can be shown $\E\left( \Phi_{k} \mid \F_{k-1} \right)= 0$, and hence $M_k = \sum_{i=0}^k \Phi_i$ is a martingale. Furthermore, we can verify $\E\norm{\Phi_k}^2 \sim \C(2\beta)$: by Cauchy-Schwarz inequality,
\begin{equation*}
    \E\norm{(k+1)^\beta x_{k+1}\zeta_k^\top}^2 \leq (k+1)^{2\beta} \sqrt{\E\norm{x_{k+1}}^4} \sqrt{\E\norm{\zeta_k}^4} \sim \C(2\beta),
\end{equation*}
where we used the result~\eqref{eq:Ex4} and the fact $\E\norm{\zeta_k}^4 = p(p+2)$. Therefore,
\begin{equation*}
\begin{aligned}
    \E\norm{\Phi_k}^2 &= \E\norm{(k+1)^\beta x_{k+1}\zeta_k^\top - H_0}^2 \leq \E \left( \norm{(k+1)^\beta x_{k+1}\zeta_k^\top} + \norm{H_0} \right)^2 \\
    & \leq 2\left( \E\norm{(k+1)^\beta x_{k+1}\zeta_k^\top}^2 + \norm{H_0}^2 \right) \sim \C( 2\beta).
\end{aligned}
\end{equation*}
By applying Lemma~\ref{lemma:martingale}, we get
\begin{equation*}
    \Hhat_{k,0} - H_0 \sim \C\left(\beta - \frac12 \right).
\end{equation*}

Now assume $\tau \geq 1$ and we already have
\begin{equation}
    \Hhat_{k,t} - H_{t} \sim \C\left(\beta - \frac12 \right)
    \label{eq:Hkt}
\end{equation}
for $t = 0,1, \ldots, \tau - 1$. Then
\begin{equation}
\begin{aligned}
&\Hhat_{k,\tau} - H_{k,\tau} \\
&= \frac{1}{k - \tau}\sum_{i=\tau + 1}^k \left\{  (i-\tau)^\beta \left[x_i - \sum_{t = 0}^{\tau - 1} \Hhat_{k, t} \ut_{i-t-1}  \right] \zeta_{i-\tau-1}^\top - H_{k,\tau} \right\} \\
&= \frac{1}{k - \tau}\sum_{i=0}^{k-\tau-1} \left\{  (i+1)^\beta \left[x_{i+\tau+1} - \sum_{t = 0}^{\tau - 1} \Hhat_{k, t} \ut_{i+\tau-t}  \right] \zeta_{i}^\top - H_{k,\tau} \right\} \\
&= \frac{1}{k - \tau}\sum_{i=0}^{k-\tau-1} \left\{  (i+1)^\beta \left[x_{i+\tau+1} - \sum_{t = 0}^{\tau - 1} H_{t} \ut_{i+\tau-t}  \right] \zeta_{i}^\top - H_{k,\tau} \right\} - \\
&\mkern108mu  \sum_{t=0}^{\tau - 1} \left( \Hhat_{k,t} - H_{t} \right) \frac{1}{k-\tau} \sum_{i=0}^{k - \tau - 1} (i+1)^\beta  \ut_{i+\tau-t}\zeta_i^\top.
\end{aligned}
\label{eq:Hktau_expanded}
\end{equation}
Completely similarly to the case $\tau = 0$, we can show
\begin{equation*}
    \frac{1}{k - \tau}\sum_{i=0}^{k-\tau-1} \left\{  (i+1)^\beta \left[x_{i+\tau+1} - \sum_{t = 0}^{\tau - 1} H_{t} \ut_{i+\tau-t}  \right] \zeta_{i}^\top - H_{k,\tau} \right\} \sim \C\left( \beta - \frac12 \right).
\end{equation*}
Meanwhile, for each of $t = 0,1,\ldots, \tau-1$, define $\Phi^t_k = (k+1)^\beta \ut_{k-t}\zeta_k^\top$. In view of~\eqref{eq:u_zeta} it can be shown $\E\left( \Phi^t_k \mid \F_{k-1} \right) = 0$, and hence $M^t_k = \sum_{i=0}^k \Phi^t_k$ is a martingale. Furthermore, in view of the fact $\norm{\ut_{k-t}}^2 \leq C^2\left(\log(k - t+1)\right)^{2} \leq C^2 \left( \log(k+1) \right)^2$, there is
\begin{equation*}
    \E\norm{\Phi^t_k}^2 \leq C^2 (k+1)^{2\beta} \left( \log(k+1) \right)^2 \E \norm{\zeta_k}^2  \sim \C(2\beta).
\end{equation*}
By applying Lemma~\ref{lemma:martingale} to $M^t_k$, we get
\begin{equation*}
    \frac{1}{k-\tau} \sum_{i=0}^{k - \tau - 1} (i+1)^\beta  \ut_{i+\tau-t}\zeta_i^\top \sim \C\left( \beta - \frac12 \right),
\end{equation*}
which together with~\eqref{eq:Hkt} implies
\begin{equation*}
  \left( \Hhat_{k,t} - H_{t} \right) \frac{1}{k-\tau} \sum_{i=0}^{k - \tau - 1} (i+1)^\beta  \ut_{i+\tau-t}\zeta_i^\top  \sim \C\left( 2\left( \beta - \frac12 \right) \right) \sim \C\left( \beta - \frac12 \right).
\end{equation*}
Now that we have shown the RHS of~\eqref{eq:Hktau_expanded} is the sum of $\tau + 1$ matrices, each of order $\C\left( \beta - \frac12 \right)$, there is
\begin{equation*}
    \Hhat_{k,\tau} - H_{k,\tau} \sim \C\left( \beta - \frac12 \right).
\end{equation*}
\end{proof}


% \begin{proof}
% As a preliminary result, notice that for any time step $k$, the variables $x_0, \zeta_0, \zeta_1, \ldots, \zeta_k, w_0, w_1, \ldots, w_k, \ut_0, \ut_1, \ldots, \ut_{k+1}$ are measurable w.r.t. $\F_k$. This together with the independence among $x_0, \zeta_0, \zeta_1, \ldots, \zeta_k, w_0, w_1, \ldots, w_k$, leads to the following relations:
% \begin{align}
%   & \E\left( \zeta_{k_1} \zeta_{k_2}^\top \mid \F_{k_2 - 1} \right) = 
%   \begin{cases} 
%     I & \text{if } k_1 = k_2 \\
%     0 & \text{otherwise},
%   \end{cases} 
%   \label{eq:zeta_zeta}
%   \\
%   & \E\left( \ut_{k_1} \zeta_{k_2}^\top \mid \F_{k_2-1} \right) = \begin{cases}
%   0 & \text{if } k_1 \leq k_2 \\
%   \text{other values} & \text{otherwise},
%   \end{cases}
%   \label{eq:u_zeta}
%   \\
%   &\E\left( w_{k_1} \zeta_{k_2}^\top \mid \F_{k_2-1} \right) = 0, 
%   \label{eq:w_zeta} \\
%   & \E\left( x_0 \zeta_{k_2}^\top \mid \F_{k_2-1} \right) = 0,
%   \label{eq:x0_zeta}
% \end{align}
% for any two time steps $k_1 \geq 0$ and $k_2 \geq 1$.

% Now let us prove the conclusion using induction on $\tau$.

% First consider the case $\tau = 0$: we have
% \begin{equation}
% \Hhat_{k,0} - H_0 = \frac1k \sum_{i=1}^k \left[(i+1)^\beta x_i \zeta_{i-1}^\top - H_0 \right]= \frac1k \sum_{i=0}^{k-1} \left( (i+2)^\beta x_{i+1} \zeta_{i}^\top - H_0\right).
% \label{eq:H0}
% \end{equation}
% Let $\Phi_k = (k+1)^\beta x_{k+1} \zeta_{k}^\top - H_0$. By substituting~\eqref{eq:static_substituted} and~\eqref{eq:zeta_zeta} to \eqref{eq:x0_zeta} into~\eqref{eq:H0} it can be shown $\E\left( \Phi_{k} \mid \F_{k-1} \right)= 0$, and hence $M_k = \sum_{i=0}^k \Phi_i$ is a martingale. Furthermore, we can verify $\E\norm{\Phi_k}^2 \sim \C(2\beta)$: by Cauchy-Schwarz inequality,
% \begin{equation}
%     \E\norm{(k+1)^\beta x_{k+1}\zeta_k^\top}^2 \leq (k+1)^{2\beta} \sqrt{\E\norm{x_{k+1}}^4} \sqrt{\E\norm{\zeta_k}^4} \sim \C(2\beta),
% \end{equation}
% where we used the result~\eqref{eq:Ex4} and the fact $\E\norm{\zeta_k}^4 = p(p+2)$. Therefore,
% \begin{equation}
% \begin{aligned}
%     \E\norm{\Phi_k}^2 &= \E\norm{(k+1)^\beta x_{k+1}\zeta_k^\top - H_0}^2 \leq \E \left( \norm{(k+1)^\beta x_{k+1}\zeta_k^\top} + \norm{H_0} \right)^2 \\
%     & \leq 2\left( \E\norm{(k+1)^\beta x_{k+1}\zeta_k^\top}^2 + \norm{H_0}^2 \right) \sim \C( 2\beta).
% \end{aligned}
% \end{equation}
% By applying Lemma~\ref{lemma:martingale}, we get
% \begin{equation}
%     \Hhat_{k,0} - H_0 \sim \C\left(\beta - \frac12 \right).
% \end{equation}

% Now assume $\tau \geq 1$ and we already have
% \begin{equation}
%     \Hhat_{k,t} - H_{t} \sim \C\left(\beta - \frac12 \right)
%     \label{eq:Hkt}
% \end{equation}
% for $t = 0,1, \ldots, \tau - 1$. Then
% \begin{equation}
% \begin{aligned}
% &\Hhat_{k,\tau} - H_{k,\tau} \\
% &= \frac{1}{k - \tau}\sum_{i=\tau + 1}^k \left\{  (i-\tau)^\beta \left[x_i - \sum_{t = 0}^{\tau - 1} \Hhat_{k, t} \ut_{i-t-1}  \right] \zeta_{i-\tau-1}^\top - H_{k,\tau} \right\} \\
% &= \frac{1}{k - \tau}\sum_{i=0}^{k-\tau-1} \left\{  (i+1)^\beta \left[x_{i+\tau+1} - \sum_{t = 0}^{\tau - 1} \Hhat_{k, t} \ut_{i+\tau-t}  \right] \zeta_{i}^\top - H_{k,\tau} \right\} \\
% &= \frac{1}{k - \tau}\sum_{i=0}^{k-\tau-1} \left\{  (i+1)^\beta \left[x_{i+\tau+1} - \sum_{t = 0}^{\tau - 1} H_{t} \ut_{i+\tau-t}  \right] \zeta_{i}^\top - H_{k,\tau} \right\} - \\
% &\mkern108mu  \sum_{t=0}^{\tau - 1} \left( \Hhat_{k,t} - H_{t} \right) \frac{1}{k-\tau} \sum_{i=0}^{k - \tau - 1} (i+1)^\beta  \ut_{i+\tau-t}\zeta_i^\top.
% \end{aligned}
% \label{eq:Hktau_expanded}
% \end{equation}
% Completely similarly to the case $\tau = 0$, we can show
% \begin{equation}
%     \frac{1}{k - \tau}\sum_{i=0}^{k-\tau-1} \left\{  (i+1)^\beta \left[x_{i+\tau+1} - \sum_{t = 0}^{\tau - 1} H_{t} \ut_{i+\tau-t}  \right] \zeta_{i}^\top - H_{k,\tau} \right\} \sim \C\left( \beta - \frac12 \right).
% \end{equation}
% Meanwhile, for each of $t = 0,1,\ldots, \tau-1$, define $\Phi^t_k = (k+1)^\beta \ut_{k-t}\zeta_k^\top$. In view of~\eqref{eq:u_zeta} it can be shown $\E\left( \Phi^t_k \mid \F_{k-1} \right) = 0$, and hence $M^t_k = \sum_{i=0}^k \Phi^t_k$ is a martingale. Furthermore, in view of the fact $\norm{\ut_{k-t}}^2 \leq C^2\left(\log(k - t+1)\right)^{2} \leq C^2 \left( \log(k+1) \right)^2$, there is
% \begin{equation}
%     \E\norm{\Phi^t_k}^2 \leq C^2 (k+1)^{2\beta} \left( \log(k+1) \right)^2 \E \norm{\zeta_k}^2  \sim \C(2\beta).
% \end{equation}
% By applying Lemma~\ref{lemma:martingale} to $M^t_k$, we get
% \begin{equation}
%     \frac{1}{k-\tau} \sum_{i=0}^{k - \tau - 1} (i+1)^\beta  \ut_{i+\tau-t}\zeta_i^\top \sim \C\left( \beta - \frac12 \right),
% \end{equation}
% which together with~\eqref{eq:Hkt} implies
% \begin{equation}
%   \left( \Hhat_{k,t} - H_{t} \right) \frac{1}{k-\tau} \sum_{i=0}^{k - \tau - 1} (i+1)^\beta  \ut_{i+\tau-t}\zeta_i^\top  \sim \C\left( 2\left( \beta - \frac12 \right) \right) \sim \C\left( \beta - \frac12 \right).
% \end{equation}
% Now that we have shown the RHS of~\eqref{eq:Hktau_expanded} is the sum of $\tau + 1$ matrices, each of order $\C\left( \beta - \frac12 \right)$, there is
% \begin{equation}
%     \Hhat_{k,\tau} - H_{k,\tau} \sim \C\left( \beta - \frac12 \right).
% \end{equation}
% \end{proof}

\renewcommand*{\proofname}{Proof}

To prove Theorem~\ref{thm:converge_J}, we identify that the suboptimality of a policy $\pi_k$ arises from three sources: i) the inaccuracy of system parameter estimates, ii) the input saturation scheme, and iii) the exploration noise. The following lemmas are meant to characterize the suboptimality caused by each of the three factors, respectively.
% They are stated without proof due to space limits.
% , and please refer to the online version of our paper~\cite{arxiv_version} for the proofs.

\paragraph*{Effect of inaccurate parameter}

The following two lemmas characterizes the sensitivity of the solution to the discrete Lyapunov equation near the optimal controller, which states the perturbation of the Lyapunov solution is quadratic in that of the feedback gain. Based on the sensitivity result, Lemma~\ref{lemma:inaccurate_param} states that the convergence speed of the control performance is twice that of the estimation error.

\begin{lemma}
Consider the discrete Lyapunov equation
\begin{align*}
    A^\top XA - X + Q = 0,
\end{align*}
where $Q$ is positive definite and $A$ is stable, then the unique positive definite solution $X$ satisfies
\begin{align*}
    \norm{X}_F \leq \norm{\left( I - A^\top \otimes A^\top \right)^{-1}}_2 \norm{Q}_F.
\end{align*}
\label{lemma:lyap_fp_norm_bound}
\end{lemma}

\begin{proof}
From the Lyapunov equation there is
\begin{align*}
    \vect(X) = \left( I - A^\top \otimes A^\top \right)^{-1} \vect(Q),
\end{align*}
and hence
\begin{align*}
    \norm{X}_F = \norm{\vect(X)}_2 \leq \norm{\left( I - A^\top \otimes A^\top \right)^{-1}}_2 \norm{\vect(Q)}_2 = \norm{\left( I - A^\top \otimes A^\top \right)^{-1}}_2 \norm{Q}_F.
\end{align*}
\end{proof}

\begin{lemma}
Let $P$ be the solution to the discrete-time algebraic Riccati equation
\begin{align*}
        P=Q+A^{\top} P A-A^{\top} P B\left(R+B^{\top} P B\right)^{-1} B^{\top} P A,
\end{align*}
and let $K$ be defined as
\begin{align*}
    K=-\left(R+B^{\top} P B\right)^{-1} B^{\top} P A.
\end{align*}
Assume $\Khat$ is such that $\tilde{A} = A + B\Khat$ is stable, and $\Phat$ satisfies the discrete Lyapunov equation
\begin{align}
    \Phat = Q + \Khat^\top R \Khat + \tilde{A}^\top \Phat \tilde{A}.
    \label{eq:lyap_Phat}
\end{align}
Let $\Delta P = \Phat - P, \Delta K = \Khat - K$, then
\begin{align*}
    \norm{\Delta P}_F \leq \norm{\left( I - \tilde{A}^\top \otimes \tilde{A}^\top \right)^{-1}}_2 \norm{R}_F \norm{\Delta K}_F^2.
\end{align*}
\label{lemma:riccati_sensitivity}
\end{lemma}

\renewcommand*{\proofname}{Proof}

% \begin{proof}
% Using the optimality of $K$, it can be shown $\Delta P$ satisfies the discrete Lyapunov equation
% \begin{align*}
%     \Delta P = \Delta K^\top R \Delta K + \tilde{A}^\top \Delta P  \tilde{A},
% \end{align*}
% and applying a bound on the norm of Lyapunov equation solution leads to the conclusion.
% \end{proof}

\begin{proof}
It can be shown $P$ satisfies the discrete Lyapunov equation
\begin{align}
    P = Q + K^\top R K + (A+BK)^\top P (A+BK).
    \label{eq:lyap_P}
\end{align}
Meanwhile, substituting $\Delta P = \Phat - P, \Delta K = \Khat - K$ into~\eqref{eq:lyap_Phat}, there is
\begin{equation}
\begin{aligned}
P + \Delta P &= Q + \left( K + \Delta K \right)^\top R \left( K + \Delta K \right) + \left( A + B \left( K + \Delta K \right) \right)^\top \left( P + \Delta P \right)\left( A + B \left( K + \Delta K \right) \right) \\
&= Q + K^\top R K + \Delta K^\top R \Delta K + (A+BK)^\top P (A+BK) + \tilde{A}^\top \Delta P  \tilde{A},
\end{aligned}
\label{eq:lyap_P_DeltaP}
\end{equation}
where for the second equality we used the fact
\begin{align*}
    \left( R + B^\top PB \right) K + B^\top PA = 0.
\end{align*}
By taking the difference between~\eqref{eq:lyap_P_DeltaP} and~\eqref{eq:lyap_P}, we can see $\Delta P$ also satisfies a discrete Lyapunov equation:
\begin{align*}
    \Delta P = \Delta K^\top R \Delta K + \tilde{A}^\top \Delta P  \tilde{A}.
\end{align*}
Applying Lemma~\ref{lemma:lyap_fp_norm_bound}, we obtain
\begin{equation*}
    \begin{aligned}
    \norm{\Delta P}_F & \leq \norm{\left( I - \tilde{A}^\top \otimes \tilde{A}^\top \right)^{-1}}_2 \norm{\Delta K^\top R \Delta K}_F \\
    & \leq \norm{\left( I - \tilde{A}^\top \otimes \tilde{A}^\top \right)^{-1}}_2 \norm{R}_F \norm{\Delta K}_F^2.
    \end{aligned}
\end{equation*}
\end{proof}


\begin{lemma}
For the system described by~\eqref{eq:dynamics} with $A$ being strictly stable and $(A,B)$ being controllable, let $J^{\pihat_k}$ be the cost defined in~\eqref{eq:J_pi} associated with the linear feedback policy $\pihat_k(x) = \Khat_k x$, where $\Khat$ is computed from estimated parameters $\Hhat_{k,\tau}$ as described in Algorithm~\ref{alg:main}, and $J^*$ be the optimal cost defined in~\eqref{eq:J_opt}, then
\begin{align*}
    % J^{\pihat_k} - J^* \sim \C\left( \alpha + \beta - \frac12 \right).
    J^{\pihat_k} - J^* \sim \C\left( 2\beta - 1 \right).
\end{align*}
\label{lemma:inaccurate_param}
\end{lemma}

% \begin{proof}
% According to Algorithm~\ref{alg:dd_lsq}, $\Ahat_k, \Bhat_k$ and hence $\Khat_k$ is differentiable w.r.t. $\Hhat_{k, \tau}$. By Lemma~\ref{lemma:function_class} and Theorem~\ref{thm:converge_H}, it follows that $\Khat_k - K \sim \C\left( \beta - \frac12 \right)$. By Lemma~\ref{lemma:riccati_sensitivity}, the convergence speed of $J^{\pihat_k}$ is twice that of $\Khat_k$, which is our conclusion.
% \end{proof}

\begin{proof}
According to the procedure described in Algorithm~\ref{alg:dd_lsq}, $\Ahat_k, \Bhat_k$ are differentiable w.r.t. $\Hhat_{k, \tau}$.
From~\eqref{eq:dare}, \eqref{eq:K}, $\Phat_k, \Khat_k$ are differentiable w.r.t. $\Ahat_k, \Bhat_k$. 
% Finally, the quadratic cost $J^{\pihat_k}$ is differentiable w.r.t. $\Khat_k$.
% The conclusion follows from Lemma~\ref{lemma:function_class} and Theorem~\ref{thm:converge_H}.
By Lemma~\ref{lemma:function_class} and Theorem~\ref{thm:converge_H}, there is
\begin{align*}
    \Khat_k - K \sim \C\left( \beta - \frac12 \right),
\end{align*}
where $K$ is the optimal gain defined in~\eqref{eq:K}.

Meanwhile, it can be shown that $J^{\pihat_k} = \Tr\left( W P_k \right)$, where $P_k$ satisfies the discrete Lyapunov equation
\begin{align*}
        P_k = Q + \Khat_k^\top R \Khat_k + \left( A + B\Khat_k \right)^\top P_k \left( A + B\Khat_k \right).
\end{align*}
Since $\Khat_k$ almost surely converges to $K$, and $A+BK$ is stable, $A+B\Khat_k$ is almost surely stable. According to Lemma~\ref{lemma:riccati_sensitivity}, it holds almost surely that
\begin{align*}
    \norm{P_k - P}_F \leq \norm{\left( I - \left( A + B\Khat_k \right)^\top \otimes \left( A + B\Khat_k \right)^\top \right)^{-1}}_2 \norm{R}_F \norm{\Khat_k - K}_F^2,
\end{align*}
where the factor $\norm{\left( I - \left( A + B\Khat_k \right)^\top \otimes \left( A + B\Khat_k \right)^\top \right)^{-1}}_2$ is bounded as $\Khat_k \to K$. Therefore, we have
\begin{align*}
    P_k - P \sim \C(2\beta - 1),
\end{align*}
and hence
\begin{align*}
    J^{\pihat_k} - J^* \sim \C\left( 2\beta - 1 \right).
\end{align*}
\end{proof}

\paragraph*{Effect of input saturation}

The following lemma follows from the observation that the tail of the $\chi^2$ distribution decays exponentially, based on which Lemma~\ref{lemma:input_sat} states that the additional cost incurred by input saturation also decays exponentially as the saturation threshold increases.

\begin{lemma}
For random variables $X\sim \chi^2(p), Y\sim \chi(p)$ and constant $M>0$, the following holds:
\begin{align}
    &\E(X-M)^+ \leq  2^{p/2+1}p \exp\left( -\frac{M}{4} \right),  \label{eq:chi2M}
    \\
    &\E\left[ (Y-M)^+ \right]^2 \leq 2^{p/2+1}p\exp\left( -\frac{M^2}{4} \right),  \label{eq:chiM}
    % &\E(X-M)^+ \leq \frac{p(p+2)}{M}, \label{eq:chi2M}\\
    % &\E\left[ (Y-M)^+ \right]^2 \leq \frac{p(p+2)}{M^2}, \label{eq:chiM}
\end{align}
where $(x)^+ \triangleq \max(x, 0)$.
\label{lemma:chiM}
\end{lemma}

% \begin{proof}
% The conclusion can be obtained by converting the expectation into a tail probability, and applying the Chernoff bound.
% \end{proof}


\begin{proof}
Let $f_{p}(x) = \frac{1}{2^{p/2} \Gamma(p/2)} x^{p/2-1}\e^{-x/2}\;(x\geq 0)$ be the probability density function of $\chi^2$ distribution with $p$ degrees of freedom. For $X\sim \chi^2(p)$, we have
\begin{equation*}
\begin{aligned}
    \E(X-M)^+ &= \int_M^\infty (x-M) f_p(x)\d x \leq \int_M^\infty xf_p(x) \d x \\
    &= \frac{2^{(p+2)/2}\Gamma\left( (p+2)/2 \right)}{2^{p/2} \Gamma(p/2)}\int_M^\infty f_{p+2}(x) \d x  \\
    % &= p P\left( \tilde{X} \geq M \right)  \leq p \frac{\E\tilde{X}}{M} = \frac{p(p+2)}{M},
    &= p P\left( \tilde{X} \geq M \right)  \leq 2^{p/2+1} p \exp\left( -\frac{M}{4} \right),
\end{aligned}
\end{equation*}
where $\tilde{X}$ is a random variable obeying $\chi^2(p+2)$, and for the last inequality we applied the Chernoff bound $P\left( X \geq M \right) \leq {\E \e^{tX}} / {\e^{tM}}$ with $t = 1/ 4$.

For $Y\sim \chi(p)$, we have
\begin{equation*}
    \begin{aligned}
    \E\left[ (Y-M)^+ \right]^2 &\leq \E\left[ (Y-M)^2 \ind{Y \geq M} \right] \leq \E\left[ \left( Y^2 - M^2 \right) \ind{Y^2 \geq M^2} \right] \\ &= \E \left( Y^2 - M^2 \right)^+ \leq 2^{p/2+1}p\exp\left( -\frac{M^2}{4} \right),
     \end{aligned}
\end{equation*}
where we noted $Y^2 \sim \chi^2(p)$ and applied~\eqref{eq:chi2M}.
\end{proof}


\input{lemma_saturation.tex}

\iffalse

\begin{lemma}
For the system described by~\eqref{eq:dynamics} with $A$ being strictly stable, let $J$ be the cost defined in~\eqref{eq:J_pi} associated with a stabilizing linear feedback policy $\pi(x) = \Khat x$, and $J^M$ be the cost associated with the ``saturated'' policy $\pi^M(x) = \proj{\Khat x}{M}$, where $\proj{v}{M}$ is defined as the projection of vector $v$ onto the Euclidean ball $\{x: \norm{x} \leq M\}$ for $M > 0$. Then
% \begin{equation}
%     J^M - J \sim \O\left( \frac{1}{M} \right)
% \end{equation}
% as $M\to\infty$.
\begin{equation*}
    J^M - J \sim \O\left( \exp\left( -cM^2 \right) \right)
\end{equation*}
as $M\to\infty$ for some constant $c>0$.
\label{lemma:input_sat}
\end{lemma}

% \begin{proof}
% Notice that all the state variables are Gaussian under the stochastically linearized closed-loop system. The conclusion can be obtained by applying an exponential tail bound of the $\chi$ distribution along with standard dynamic programming arguments.
% \end{proof}


\begin{proof}
We may first consider the finite horizon cost
\begin{align*}
    J^\pi_T = &  \E\left[ \sum_{k=0}^{T-1} x_k^\top Q x_k + u_k^\top R u_k \right], \\
    & \text{where } x_0 \sim \gaussian{0}{X_0}, u_k = \pi\left( x_k \right), x_{k+1} \text{ satisfies~\eqref{eq:dynamics}},
\end{align*}
and take the limit as $T\to\infty$ to get the desired result.

Let us define the finite horizon values functions of policies $\pi$ and $\pi^M$ as
\begin{align*}
    & V_T(x) = x^\top Qx, \\
    & V_t(x) = x^\top Qx + \pi(x)^\top R \pi(x) + \E V_{t+1}\left( Ax + B\pi(x) + w_t \right),\; t = 0,1,\ldots,T-1, \\
    & V^M_T(x) = x^\top Qx, \\
    & \begin{aligned} V^M_t(x) = x^\top Qx + \pi^M(x)^\top R \pi^M(x) + \E V^M_{t+1}\left( Ax + B\pi^M(x) + w_t \right),\\ t = 0,1,\ldots,T-1. \end{aligned}
\end{align*}
Then the finite horizon costs of policies $\pi$ and $\pi^M$ can be represented as
\begin{align*}
    J_T = \E V_0\left( x_0 \right), J^M_T = \E V^M_0\left( x_0 \right),
\end{align*}
and we have
\begin{align*}
    J^M - J = \lim_{T\to\infty} \frac 1T \left( J^M_T - J_T \right)
\end{align*}
provided the limit exists. Next we will attempt to bound $J_T^M - J_T$ in terms of $M$.

We first notice that $V_t$ is a quadratic function of $x$, which we denote by
\begin{align}
    V_t(x) = x^\top \Phat_t x + \qhat_t, \label{eq:V_explicit}
\end{align}
where $\Phat_t, \qhat_t$ satisfy the recursion formulas
\begin{align*}
    & \Phat_T = Q, \Phat_t = Q + \Khat^\top R \Khat + \left( A + B\Khat \right)^\top \Phat_{t+1} \left( A + B\Khat \right)\; t = 0,1,\ldots, T-1, \\
    & \qhat_T = 0, \qhat_t = \qhat_{t+1} + \Tr(W\Phat_{t+1}),\; t = 0,1,\ldots, T-1.
\end{align*}
Since $A+B\Khat$ is strictly stable, we have
\begin{align}
    \sup_{T > 0} \max_{t=0,1,\ldots, T} \norm{\Phat_t} < \infty.
    \label{eq:Phat_bound}
\end{align}

To simplify notations, let us define
\begin{align*}
    &\DVtot_t(x) = V^M_t(x) - V_t(x), \\
    &\DVstep_t(x) = V_{t+1}\left( Ax + B\pi^M(x) \right) - V_{t+1}\left( Ax + B\pi(x) \right), \\
    &\Dpi(x) = \pi^M(x) - \pi(x),
\end{align*}
then $J_T^M - J_T = \E \Delta_0\left( x_0 \right)$, and we have the following recursion formula:
\begin{equation*}
\begin{aligned}
    \DVtot_T(x) &= 0, \\
    \DVtot_t(x) &\leq \E\left[ V^M_{t+1}\left( Ax + B\pi^M(x) + w_t \right) - V_{t+1}\left( Ax + B\pi(x) + w_t \right) \right] \\
    &= \E\left[ V^M_{t+1}\left( Ax + B\pi^M(x) + w_t \right) \right] - \E\left[ V_{t+1}\left( Ax + B\pi^M(x) + w_t \right) \right] + \\
    &\mkern48mu \E\left[ V_{t+1}\left( Ax + B\pi^M(x) + w_t \right) \right] - \E\left[ V_{t+1}\left( Ax + B\pi(x) + w_t \right) \right] \\
    &= \E \DVtot_{t+1} \left( Ax + B\pi^M(x) + w_t \right) + \DVstep_t(x),\quad t = 0,1,\ldots, T-1,
\end{aligned}
\end{equation*}
where for the first equality we noted the fact $\pi^M(x)^\top R \pi^M(x) \leq \pi(x)^\top R \pi(x)$, and for the last equality
% we noticed that $\pi(x) = \Khat x$ is a linear feedback policy, and it can be shown
% \begin{align}
%   \E V_{t+1}\left( Ax + B\pi(x) + w_t \right) = V_{t+1}\left( Ax + B\pi(x)  \right) + \Tr(QW) .
%   \label{eq:trqw}
% \end{align}
we applied~\eqref{eq:V_explicit}. Hence,
\begin{equation}
\begin{aligned}
    \E \DVtot_t(x) \leq & \E \DVtot_{t+1}\left( A + B\pi(x) + w_t \right) + \underbrace{\E \DVstep_t(x)}_{\text{I}} + \\ & \underbrace{\E \left[ \DVtot_{t+1}\left( Ax + B\pi^M(x) + w_t \right)-\DVtot_{t+1}\left( Ax + B\pi(x) + w_t \right) \right]}_{\text{II}}.
\end{aligned}
\label{eq:DVtot_expanded}
\end{equation}
Now we assume $x\sim \gaussian{0}{X}$ and bound the terms I and II respectively. For I, we have
\begin{align}
    \DVstep_t(x) = 2 \Dpi(x)^\top B^\top \Phat_{t+1} \left( A + B\Khat \right) x + \Dpi(x)^\top \Phat_{t+1} \Dpi(x).
    \label{eq:DVstep_expanded}
\end{align}
Since
\begin{align*}
    \norm{\Dpi(x)} = \max\left( \norm{\pi(x)} - M, 0 \right)
\end{align*}
and
\begin{align*}
    \norm{\left( \Khat X \Khat^\top \right)^{-1/2} \pi(x)} \sim \chi(m),
\end{align*}
in view of Lemma~\ref{lemma:chiM}, \eqref{eq:Phat_bound} and the stability of $A + B\Khat$, we have
\begin{align}
    % \E \DVstep_t(x) \sim \O\left( \frac{\norm{X}}{M} \right).
    \E \DVstep_t(x) \sim \O\left( \norm{X} \exp\left( -\frac{M^2}{8\norm{X}\norm{\Khat}^2} \right) \right).
    \label{eq:DVstep_bound}
\end{align}
For II, consider $\DVtot_t(\xi + \delta) - \DVtot_t(\xi)$ for any $\xi,\delta \in \R{n}$: we have
\begin{align*}
    \DVstep_t(\xi + \delta) - \DVstep_t(\xi) \sim \O \left( \norm{\xi}\norm{\delta}^2\norm{\xi + \delta} \right)
\end{align*}
due to~\eqref{eq:DVstep_expanded} and the fact
\begin{align*}
    \norm{\Dpi(\xi + \delta) - \Dpi(\xi)} \leq 2 \norm{\Khat}\norm{\delta}.
\end{align*}
It follows that
\begin{align*}
    \DVtot_{T-1}(\xi + \delta) - \DVtot_{T-1}(\xi) = \DVstep_{T-1}(\xi + \delta) - \DVstep_{T-1}(\xi) \sim \O \left( \norm{\xi}\norm{\delta}^2\norm{\xi + \delta} \right).
\end{align*}
Therefore,
\begin{equation*}
\begin{aligned}
    & \DVtot_{T-2}(\xi + \delta) - \DVtot_{T-2}(\xi) \\
    = & \E\left[ \DVtot_{T-1}\left( \xi^+ + \delta^+ \right) - \DVtot_{T-1}\left( \xi^+ \right) \right] + \DVstep_{T-2}(\xi + \delta) - \DVstep_{T-2}(\xi) \\
    \sim & \O \left( \left( 1+\rho^2 \right) \norm{\xi}\norm{\delta}^2\norm{\xi + \delta} \right),
\end{aligned}
\end{equation*}
where $\xi^+ = A\xi + B\pi^M(\xi) + w_t, \delta^+ = A\delta + B \left( \pi^M(\xi+\delta) - \pi^M(\xi) \right)$, and $\rho = \max\left( \rho(A), \rho\left( A + B\Khat \right) \right) < 1$.
In a similar manner, it can be shown
\begin{align*}
    \DVtot_{T-t}(\xi+\delta) - \DVtot_{T-t}(\xi) \sim \O \left( \left(1+\rho^2 + \cdots + \rho^{2(t-1)}\right)  \norm{\xi}\norm{\delta}^2\norm{\xi + \delta} \right)
\end{align*}
for $t=0,1,\ldots, T-1$. Therefore,
\begin{align*}
    \DVtot_t(\xi+\delta) - \DVtot_t(\xi) \sim \O\left( \left( 1 - \rho^2 \right)^{-1} \norm{\xi}\norm{\delta}^2\norm{\xi + \delta} \right) \sim \O\left(  \norm{\xi}\norm{\delta}^2\norm{\xi + \delta} \right), 
\end{align*}
which does not depend on $T$. Substituting in $\xi = Ax + B\pi(x) + w_t$ and $\delta = \Dpi(x)$, and taking the expectation, it can be shown
\begin{align}
    \E \left[ \DVtot_{t+1}\left( Ax + B\pi^M(x) + w_t \right)-\DVtot_{t+1}\left( Ax + B\pi(x) + w_t \right) \right] \sim \O\left( \norm{X} \exp\left( -\frac{M^2}{8\norm{X}\norm{\Khat}^2} \right) \right).
    \label{eq:DVtot_diff_bound}
\end{align}
Finally, we substitute~\eqref{eq:DVstep_bound} and \eqref{eq:DVtot_diff_bound} back into~\eqref{eq:DVtot_expanded} and notice that when $x \sim \gaussian{0}{X}$, there is
\begin{align*}
    A + B\pi(x) + w_t \sim \gaussian{0}{\left( A + B\Khat \right) X \left( A + B\Khat \right)^\top + W},
\end{align*}
and the covariance is bounded as $T\to\infty$ due to the strict stability of $A + B\Khat$. Therefore, we have
\begin{align*}
    J_T^M - J_T = \E \DVtot_0(x_0) \sim \O\left( T \exp\left( -cM^2 \right) \right),
\end{align*}
which implies our conclusion.
\end{proof}

\fi

\paragraph*{Effect of exploration noise}

The following lemma is based on the observation that the exploration noise affects the cost in terms of i) changing the system dynamics, and ii) increasing the $u_k^\top R u_k$ terms in the cost, and each of the effects is of the same order as the noise covariance.

\begin{lemma}
For the system described by~\eqref{eq:dynamics}, let $J$ be the cost defined in~\eqref{eq:J_pi} associated with a stabilizing linear feedback policy $\pi(x) = \Khat x$, and $J^\Zeta$ be the cost defined in~\eqref{eq:J_pi} associated with the corresponding ``noisy'' policy $\pi^\Zeta(x) = \Khat(x) + \zeta,\ \zeta \sim \gaussian{0}{\Zeta}$, then as $\Zeta \to 0$,
\begin{align*}
    J^\Zeta - J \sim \O \left( \norm{\Zeta} \right).
\end{align*}

\label{lemma:input_noise}
\end{lemma}

% \begin{proof}
% The additional noise input affects the cost in terms of i) changing the dynamics of the system; ii) increasing the $u_k^\top R u_k$ terms in the cost. The former can be equivalently seen as increasing the process noise covariance by $\Zeta$, and the cost induced by the latter is $\Tr(\Zeta R) \sim \O\left( \norm{\Zeta} \right)$. Superposing the two effects leads to the conclusion.
% \end{proof}

\begin{proof}
Denote by $J^\Zeta_W$ the cost associated with policy with input noise covariance $\Zeta$, acting on open-loop system with process noise covariance $W$. Then $J^\Zeta = J^\Zeta_W$, and $J = J^0_W$. Next we will bound $J^Z_W - J^0_{Z+W}$ and $J^0_{Z+W} - J^0_{W}$.

Notice that $J^\Zeta_W$ and $J^0_{Z+W}$ are associated with the same closed-loop system, and only differ in the $u_k^\top R u_k$ term in the cost. It can be shown
\begin{align}
    J^\Zeta_W - J^0_{Z+W} = \Tr(\Zeta R) \sim \O\left( \norm{\Zeta} \right).
\end{align}
Meanwhile, for an arbitrary process noise covariance matrix $W$, we have
\begin{align}
J^0_W = \lim_{T\to\infty}\frac 1T\E V_0(x),
\label{eq:cost_diff}
\end{align}
where
\begin{align}
    V_t(x) = x^\top \Phat_t x + \qhat_t,
\end{align}
and $\Phat_t, \qhat_t$ satisfy the recursion formulas
\begin{align}
    & \Phat_T = Q, \Phat_t = Q + \Khat^\top R \Khat + \left( A + B\Khat \right)^\top \Phat_{t+1} \left( A + B\Khat \right)\; t = 0,1,\ldots, T-1, \\
    & \qhat_T = 0, \qhat_t = \qhat_{t+1} + \Tr(WP_{t+1}),\; t = 0,1,\ldots, T-1.
\end{align} 
Since $\Khat$ is stabilizing, it can be shown $\Phat_0 \to \Phat$ for some bounded $\Phat$ as $T\to\infty$ which is independent of $W$, and hence
\begin{align}
    J^0_{\Zeta+W} - J^0_{W} = \Tr\left( \Zeta \Phat \right) \sim \O\left( \norm{\Zeta} \right).
\label{eq:dyn_diff}
\end{align}
The conclusion follows from~\eqref{eq:cost_diff} and~\eqref{eq:dyn_diff}.
\end{proof}

Finally, a combination of Lemmas~\ref{lemma:inaccurate_param}, \ref{lemma:input_sat}, and \ref{lemma:input_noise} leads to Theorem~\ref{thm:converge_J}.

% By combining Lemmas~\ref{lemma:inaccurate_param}, \ref{lemma:input_sat} and \ref{lemma:input_noise}, we are ready to prove Theorem~\ref{thm:converge_J}.

\renewcommand*{\proofname}{Proof of Theorem~\ref{thm:converge_J}}

\begin{proof}
Denote the policies by $\pihat_k(x) = \Khat_k x$, $\pit_k(x) = \proj{\Khat_k x}{C\log(k+1)}$, $\pi_k(x) = \proj{\Khat_k x}{C\log(k+1)} + k^{-\beta}\zeta, \zeta \sim \gaussian{0}{I_p}$. Similarly as in the proof of Lemma~\ref{lemma:input_noise}, we notice the closed-loop system of $\pi_k$ acting on the original system is equivalent to the closed-loop system of $\pit_k$ acting on a system with process noise covariance $W+k^{-\beta}I$, and the cost of the two cases differ by $\O(-\beta)$. By Lemma~\ref{lemma:input_sat}, the cost of $\pit_k$ and $\pihat_k$ on the system differ by $\O\left( \exp\left( -ck^2 \right) \right) \sim \C(0)$. Since $\pihat_k$ is a linear feedback policy, similarly as in the proof of Lemma~\ref{lemma:input_noise}, the cost of $\pihat_k$ on the systems with process noise covariance $W+k^{-\beta}I$ and $W$ differ by $\O(-\beta)$. Finally, on the original system, by Lemma~\ref{lemma:inaccurate_param}, the cost of $\pihat_k$ and the optimal policy differ by $\C(-2\gamma)$. By summing up the above terms, we get $J^{\pi_k} - J^* \sim \C\left( -\min(0, \beta, 2\gamma)\right) = \C\left( -\min(\beta, 2\gamma)\right)$.
\end{proof}

==> figures/simulation.tex <==
\section{Simulation}\label{sec:simulation}

In this section, the performance of our proposed algorithm is evaluated using Tennessee Eastman Process~(TEP), an industrial process example for benchmarking linear controllers~\citep{tep}. We used a simplified version of TEP from~\cite{watermark}, where the state and input dimensions are $n = 8, p = 4$, and the spectral radius of the system matrix is $\rho(A) \approx 0.96$. We assume $Q,R,W,X_0$ are identity matrices with proper dimensions. We choose $N = 50$ (in Algorithm~\ref{alg:dd_lsq}) for all the experiments.
In the practical implementation, the estimated system matrices $\Ahat_k, \Bhat_k$ and the feedback gain $\Khat_k$ are updated only at steps $\lfloor 10^{n/2} \rfloor (n\in\mathbb{N}) $ to speed up the computation.
% When implementing Algorithm~\ref{alg:main}, we made the observation that the convergence of parameter estimates does not rely on a particular control policy, as long as the policy is stabilizing in the limit sense. Therefore, in our implementation, the estimated system matrices $\Ahat_k, \Bhat_k$ and the feedback gain $\Khat_k$ are updated once per 1000 steps to in order to speed up the computation.

To illustrate the impact of the parameter $\beta$ on the convergence of the algorithm, we perform 100 independent experiments for each of $\beta \in \left\{ 0, 1/4, 1/2 \right\}$, with $10^8$ steps in each experiment. 
Fig.~\ref{fig:converge_param} shows the error of the estimated system and input matrices, i.e., $\norm{\Ahat_k - A}$ and $\norm{\Bhat_k - B}$ against the time $k$ for different values of $\beta$.

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/Ahat.tikz}
    \end{subfigure} \hfill
    \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/Bhat.tikz}
    \end{subfigure}
    \caption{Error of estimated system matrices for different $\beta$ against time $k$. The solid lines are the median among the experiments, and the shades represent the range among the experiments.}
    \label{fig:converge_param}
\end{figure}

From Fig.~\ref{fig:converge_param}, one can see when $\beta$ is $0$ or $1/4$, the estimation error of the system matrices converges to zero as time $k$ goes to infinity, and the convergence approximately follows a power law. Furthermore, the convergence speed of the estimation error is significantly faster when $\beta = 0$. Meanwhile, when $\beta = 1/2$, the estimate error diverges in some of the experiments. The above observations are consistent with the theoretical result in Theorem~\ref{thm:converge_H}, where it is stated that the parameter estimates converge with rate $\O\left( k^{-\gamma + \epsilon} \right)$, with $\gamma = 1/2 - \beta$, i.e., convergence is only guaranteed with $\beta < 1/2$ and is faster when $\beta$ is smaller.

% Fig.~\ref{fig:percentage_stabilizing} shows how many out of the 100 experiments find stabilizing controllers as time evolves for different values of $\beta$. Since the $A$ is already stable, and $\Khat_0 = 0$, the controllers are stabilizing in the initial stage. As $k$ increases, the algorithm consistently finds stabilizing controllers when $\beta = 0$, the case when the convergence of parameter estimates is the fastest. When $\beta = 1/3$, the system is destabilized in a few experiments when $k$ is relatively small but is consistently stabilized after $10^5$ steps. When $\beta = 1/2$, the system is destabilized in a significant portion of the experiments and is still not always stabilized after $10^6$ steps. This observation is consistent with the theoretical analysis that the algorithm is valid only when $\beta < 1/2$.

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/percentage_stabilizing_bar.tikz}
%     \caption{Percentage of experiments finding stabilizing controllers for different $\beta$ against time $k$. The controller at step $k$ is stabilizing when $\rho\left( A + B \Khat_k \right) < 1$. For each $k \in \left\{10^0, 10^1, \ldots,10^6 \right\}$, the bars show how many of the 100 experiments find stabilizing controllers at step $k$.}
%     \label{fig:percentage_stabilizing}
% \end{figure}
Now we consider the performance of policies with different values of $\beta$.
To quantify the policy performance, one shall in theory compute $J^{\pi_k}$ as defined in~\eqref{eq:J_pi}. However, the policies $\pi_k$ are nonlinear, rendering it very difficult, if not impossible, to compute $J^{\pi_k}$ analytically. As a surrogate approach for evaluating a policy $\pi_k$, we define the empirical cost $\hat{J}^{\pi_k}$ as
\begin{equation*}
    \hat{J}^{\pi_k} = \frac{1}{N}\frac{1}{T}\sum_{i=1}^N\sum_{t=0}^{T-1} \left( x_t^{(i)} \right)^\top Q x_t^{(i)} + \left( u_t^{(i)} \right)^\top R u_t^{(i)},
\end{equation*}
where $x_t^{(i)}, u_t^{(i)}$ are states and inputs collected from the closed-loop system under $\pi_k$ in $N$ independent $T$-long sample paths indexed by $i$. In our simulations, we take $T = 10000, N = 10$ to evaluate each stabilizing policy, which yields consistent results in practice. Fig.~\ref{fig:J} shows the empirical performance of controllers with different values of $\beta$ against time $k$.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/J.tikz}
    \caption{The empirical performance of controllers for different $\beta$ against time $k$. For each policy $\pi_k$, the empirical cost $\hat{J}^{\pi_k}$ is obtained by approximating the actual cost with random sampling from the closed-loop system. The solid lines are the median among the experiments, and the shades represent the interval between the first and third quantiles among the experiments. The purple and brown dashed lines represent the analytical optimal cost, and the analytical cost of the control-free system, respectively.}
    \label{fig:J}
\end{figure}

From Fig.~\ref{fig:J}, one can observe that among our choices of $\beta$, only $\beta = 1/4$ drives the controller toward the optimal one. For $\beta = 0$, although the parameter estimates converge the fastest as discussed above, the performance of the resulting closed-loop system is even worse than the free system. This is because the exploration term $(k+1)^{-\beta}\zeta_k$ in the control input does not decay, and the resulting controller is a noisy one. Meanwhile, for $\beta = 1/2$, diverging parameter estimates would lead to ill-performing controllers. The observations are consistent with the theoretical conclusion indicated by Theorem~\ref{thm:converge_J} that $\beta = 1/4$ corresponds to the optimal trade-off between exploration and exploitation.

\revise{
    Finally, we compare our algorithm with the naive centainty equivalence algorithm, which applies $u_k = \Khat_k x_k$ at each step. We invoke both algorithms with the ``optimal'' parameter $\beta = 1/4$.

    \begin{figure}[!htbp]
        \centering
        \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/Ahat_ce.tikz}
        \end{subfigure} \hfill
        \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/Bhat_ce.tikz}
        \end{subfigure} \hfill
        \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/J_ce.tikz}
        \end{subfigure}
    \end{figure}
}

==> lemma_saturation.tex <==
\begin{lemma}
For the system described by~\eqref{eq:dynamics} with $A$ being strictly stable, let $J$ be the cost defined in~\eqref{eq:J_pi} associated with an arbitrary stabilizing linear feedback policy $\pi(x) = \Khat x$, and $J^M$ be the cost associated with the ``safe'' policy $\pi^M(x;\safesteps) = {\Khat x}\ind{\safesteps=0},\safesteps \gets \begin{cases}t & \norm{x} > M \\ \max(\safesteps - 1, 0) & \text{otherwise}\end{cases}$.
Then there is
\begin{equation}
    J^M - J \sim \O\left( \frac{t}{M^2} \right)
\end{equation}
as $M\to\infty, t\to\infty, M^2/t\to\infty$.
% \begin{equation*}
%     J^M - J \sim \O\left( \exp\left( -cM^2 \right) \right)
% \end{equation*}
% as $M\to\infty$ for some constant $c>0$.
\label{lemma:input_sat}
\end{lemma}

\begin{proof}
Because $A+B\Khat$ is stable, for any fixed matrix $Q > 0$, the Lyapunov equation $\left(A+B\Khat\right)^\top P \left(A+B\Khat\right) + Q = P$ has a solution $P > 0$. Therefore, there exists a matrix $P>0$ and a scalar $0 < \rho < 1$, such that $\left(A+B\Khat\right)^\top P \left(A+B\Khat\right) < \rho P$. Furthermore, because $A$ is stable, there is $A^t \to 0$ as $t\to \infty$, and therefore, for any matrix $P>0$ and scalar $0 < \rho < 1$, assuming $t$ is sufficiently large, there is $\left(A^t\right)^\top P A^t < \rho P$.

Now assuming both $\left(A+B\Khat\right)^\top P \left(A+B\Khat\right) < \rho P$ and $\left(A^t\right)^\top P A^t < \rho P$, where $P>0, 0<\rho <1$, we define the Lyapunov function $V(x) = x^\top P x$. Then, \begin{itemize}
    \item If $\norm{x_k} < M$, there is
    \begin{align}
        \E\left[ V\left( x_{k+1} \right) \mid \F_k\right] &= x_k^\top \left(A+B\Khat\right)^\top P \left(A+B\Khat\right) \leq \rho V\left( x_k \right) + \Tr(WP),
        \label{eq:condexp_lyap_1}
    \end{align}
    \item If $\safesteps = 0$ at step $k$ and $\norm{x_k} \geq M$, there is
    \begin{align}
    \begin{aligned}
        \E\left[ V\left( x_{k+t} \right) \mid \F_k\right] &=
        \E\left[ \left( A^tx_k + A^{t-1}w_k + \cdots + w_{k+1-1} \right)^\top P \left( A^tx_k + A^{t-1}w_k + \cdots + w_{k+1-1} \right) \mid \F_k \right] \\
        &= x_k^\top \left(A^t\right)^\top P A^t x_k + \Tr\left( W \left( \left( A^{t-1} \right)^\top P A^{t-1} + \cdots + A^\top PA + P \right) \right)\\
        & \leq \rho V\left(x_k\right) + \Tr\left(W\Pt\right),
    \end{aligned}
        \label{eq:condexp_lyap_2}
    \end{align}
    where we define $\Pt \triangleq \lim_{t\to\infty} \left( A^{t-1} \right)^\top P A^{t-1} + \cdots + A^\top PA + P$.
\end{itemize}

To unify the above two cases, let us define the process $\left\{ \xt_k \right\}$ as follows: $\xt_k = x_{i(k)}$, where $i(0) = 0, i(k+1) = \begin{cases} i(k)+1 & \norm{x_{i(k)}} < M \\ i(k)+t & \norm{x_{i(k)}} \geq M \end{cases}$. That is, $\left\{ \xt_k \right\}$ is a subsequence of $\left\{ x_k \right\}$, in which the steps where $0<\safesteps<t$ are skipped. By combining~\eqref{eq:condexp_lyap_1} and~\eqref{eq:condexp_lyap_2}, we get
\begin{align}
    \E\left[ V\left( \xt_{k+1} \right) \mid \Ft_k \right] \leq \rho V\left( \xt_k \right) + c,
    \label{eq:condexp_lyap_unified}
\end{align}
where $\Ft_k = \F_{i(k)}$, and $c = \Tr\left( W\Pt\right)$ is a constant.

Now let $V_k = V\left( \xt_k \right)$ and $U_k = \rho^{-k}\left( V_k - \frac{c}{1 - \rho}\right)$, and then it follows from~\eqref{eq:condexp_lyap_unified} that $\E\left[ U_{k+1} \left| \Ft_k \right. \right] \leq U_k$, i.e., $\left\{ U_k \right\}$ is a supermartingale adapted to the filtration $\left\{ \Ft_k \right\}$. We will proceed in three steps: i) bounding the escape probability of $U_k$, and hence of $V_k$ and $\norm{\xt_k}$; ii) showing the boundedness of $\E V_k^2$, and hence of $\E\norm{\xt_k}^4$ and $\E \norm{x_k}^4$; iii) bounding $J^M-J$ by comparing the trajectories of the systems driven by $\pi^M$ and $\pi$ respectively.

For the first step, we apply Doob's maximal inequality to the supermartingale $\left\{ U_k \right\}$: for any $N>0$, there is
\begin{align*}
    P\left( \sup_{0\leq s \leq k} U_s \geq N \right) &\leq P\left( \sup_{0\leq s \leq k} \left| U_s\right| \geq N \right)
    \leq \frac{\E U_0 + 2\E\left( U_k^- \right)}{N} \leq \frac{\Tr\left( X_0P\right) + 2\frac{c}{1 - \rho}}{N}
\end{align*}
for any $k$, where $U_k^-$ denotes the negative part of $U_k$.
Hence, for any $N > \frac{c}{1 - \rho}$, we have
\begin{align*}
    P\left( V_k \geq N \right) = P \left( U_k \geq \rho^{-1} \left( N - \frac{c}{1 - \rho} \right) \right) \leq \frac{\rho^k}{N - \frac{c}{1 - \rho}}.
\end{align*}
In the asymptotic notation, this is $P\left(V_k \geq N \right) \sim \O\left(\rho^k / N \right)$ as $N\to\infty$, and therefore $P\left(\norm{x_k} \geq M \right) \sim \O\left(\rho^{k} / M^2\right)$ as $M \to\infty$.
% This implies $P\left(U_k \geq N \right) \sim \O(1/N)$, and hence $P\left(V_k \geq N \right) \sim \O\left(\rho^k / N \right)$ and $P\left(\norm{x_k} \geq M \right) \sim \O\left(\rho^{k} / M^2\right)$.

For the second step, to prove $\E V_k^2$ is bounded, it suffices to prove $\E U_k^2  \sim \O\left(\rho^{-2k}\right)$. In view of the equality $U_{k+1}^2 = U_k^2 + U_{k+1}\left(U_{k+1} - U_k\right) + U_{k}\left(U_{k+1} - U_k\right)$, we can inspect to last two terms respectively. By the definition of $U_k$, there is
\begin{align}
U_{k+1}\left(U_{k+1} - U_k\right) = \rho^{2k-2} \left[ V_{k+1}^2 - \left( \rho V_k + c + \frac{c}{1-\rho}\right) V_{k+1} + \frac{c}{1-\rho}\left(\rho V_k + c\right)\right],
\label{eq:U_Udiff}
\end{align}
and by the definition of $V_k$, there is
\begin{align*}
V_{k+1} &= \xt_{k+1}^\top P\xt_{k+1} = \left(\At_k \xt_k + \wt_k\right)^\top P \left(\At_k \xt_k + \wt_k\right) \leq \rho V_k + \xi_k,
\end{align*}
where
\begin{itemize}
    \item $\At_k \in \left\{ A+B\Khat, A^t \right\}$ and it follows that $\At_k^\top P \At < \rho P$;
    \item $\wt_k$ is either $w_{i(k)}$ or the weighted sum of $t$ independent Gaussian random vectors $w_{i(k)}, \ldots, w_{i(k+t-1)}$, and therefore has finite moments of all orders;
    \item $\xi_k = 2\xt_k \At_k^\top P \wt_k + \wt_k^\top P \wt_k$, from which it follows that $\E\left[\xi_k^2 \left| \Ft_k \right. \right] \sim \O\left(\norm{\xt_k}^2\right) \sim \O \left( V_k \right)$ and $\E\left[\xi_k^4 \left| \Ft_k\right. \right] \sim \O\left(\norm{\xt_k}^4\right) \sim \O\left( V_k ^2 \right)$.
\end{itemize}
Meanwhile, from the above definition of $\xi_k$, there is also $V_{k+1} \geq \xi_k$ since $\At_k^\top P \At_k \geq 0$. Combining $\xi_k \leq V_{k+1} \leq \xi_k + \rho V_k$ with~\eqref{eq:U_Udiff}, and using the fact that the RHS of~\eqref{eq:U_Udiff} is a convex quadratic function of $V_{k+1}$, we get
\begin{align*}
\begin{aligned}
    \E \left[ U_{k+1}\left(U_{k+1}  - U_k\right)\left| \Ft_k \right. \right] &\leq \rho^{2k-2} \E \left[\max \left\{ \xi_k^2 - \left( \rho V_k + c + \frac{c}{1-\rho}\right) \xi_k + \frac{c}{1-\rho}\left(\rho V_k + c\right),\right.\right. \\& \left.\left.\left. \left(\xi_k + \rho V_k\right)^2 - \left( \rho V_k + c + \frac{c}{1-\rho}\right) \left(\xi_k + \rho V_k\right) + \frac{c}{1-\rho}\left(\rho V_k + c\right)  \right\} \right| \Ft_k \right]
    \\
    & \leq \rho^{2k-2} \left( \sqrt{\E\left[ \left. \left( \xi_k^2 - \left( \rho V_k + c + \frac{c}{1-\rho}\right) \xi_k + \frac{c}{1-\rho}\left(\rho V_k + c\right) \right)^2 \right| \Ft_k\right]}\right. \\&+\left. \sqrt{\E\left[ \left. \left( \left(\xi_k + \rho V_k\right)^2 - \left( \rho V_k + c + \frac{c}{1-\rho}\right) \left(\xi_k + \rho V_k\right) + \frac{c}{1-\rho}\left(\rho V_k + c\right) \right)^2 \right| \Ft_k\right]} \right) \\
    & \sim \O \left( \rho^{2k} V_k^2 \right),
\end{aligned}
\end{align*}
where for the second inequality we used the fact that $\E \left[\max\{ f(x), g(x) \}\right] = \E\left[ f(x) \ind{f(x) \geq g(x)}\right] + \E \left[ g(x) \ind{f(x) < g(x)} \right] \leq \sqrt{\E f(x)^2} + \sqrt{\E g(x)^2}$ provided all these expectations exist. In a similar manner, it can be shown
\begin{align*}
    \E \left[ U_k(U_{k+1}-U_k) \left| \Ft_k \right. \right] &=  \E \left[\left. \rho^{2k-1} \left( V_k - \frac{c}{1 - \rho}\right) (V_{k+1} - \rho V_k - c) \right| \Ft_k  \right] \\
    &\leq \rho^{2k-1} \E \left[\left. \max\left\{\left( V_k - \frac{c}{1 - \rho}\right)(\xi_k - \rho V_k - c), \left( V_k - \frac{c}{1 - \rho}\right)(\xi_k - c)  \right\} \right| \Ft_k \right] \\
    &\leq \rho^{2k-1} \left(  \E\left[ \left. \left( V_k - \frac{c}{1 - \rho}\right)(\xi_k - \rho V_k - c) \right| \Ft_k \right]  + \E\left[ \left. \left( V_k - \frac{c}{1 - \rho}\right)(\xi_k - c) \right| \Ft_k \right]  \right) \\
    & \sim \O\left( \rho^{2k} V_k^2 \right).
\end{align*}
Now we can prove $\E U_k^2  \sim \O\left(\rho^{-2k}\right)$ by induction: assuming $\E U_k^2 \leq M_1\rho^{-2k}$, and that
$\E \left[ U_{i+1}\left(U_{i+1}  - U_i\right)\left| \Ft_i \right. \right] 
\leq M_2 \rho^{2i}V_i^2, \E \left[ U_{i}\left(U_{i+1}  - U_i\right)\left| \Ft_i \right. \right] 
\leq M_2 \rho^{2i}V_i^2$ for any $i$, then $\E V_k^2 = \E \left( \rho^k U_k + \frac{c}{1 - \rho}\right)^2 \leq M_1 + \frac{2c}{1-\rho}\sqrt{M_1} + \left(\frac{c}{1 - \rho}\right)^2 \leq 2M_1$, provided $M_1$ is sufficiently large. Therefore,
\begin{align*}
    \E U_{k+1}^2 &= \E U_k^2 + \E\left[\E \left[ U_{k+1}\left(U_{k+1}  - U_k\right)\left| \Ft_k \right. \right]\right] + \E\left[\E \left[ U_{k}\left(U_{k+1}  - U_k\right)\left| \Ft_k \right. \right]\right] \\
    &\leq \rho^{-2k} M_1 \left(1 + 4M_2 \rho^{2k} \right) \leq \rho^{-2k-2} M_1,
\end{align*}
provided $k$ is sufficiently large. Therefore, we have $\E U_k^2  \sim \O\left(\rho^{-2k}\right)$, and hence $\E\left(\xt_k^\top P \xt_k \right)^2 = \E V_k^2 \sim \O(1)$, i.e., $\E \norm{\xt_k}^4 \sim \O(1)$.

To establish the relationship between $\E \norm{\xt_k}^4$ and $\E\norm{x_k}^4$, notice that
\begin{align*}
    x_k = A^{k - i(j)} \xt_j + \sum_{l=0}^{k - i(j) - 2} A^{k - i(j) - 1 - l}w_{j+l},
\end{align*}
where $j$ is defined as $j = \sup\left\{ s \mid s\in \mathbb{Z}^+, i(s) \leq k \right\}$, i.e., $\xt_j$ is the state in $\left\{ \xt_k \right\}$ that physically occurs no later than $x_k$. Since $A$ is stable and $\{w_k \}$ are i.i.d Gaussian, $\E \norm{\xt_k}^4 \sim \O(1)$ implies $\E \norm{x_k}^4 \sim \O(1)$.

For the final step, let $\left\{ \xhat_k \right\}$ denote the state trajectory driven by $\pi$, and $\left\{ x_k \right\}$ denote the state trajectory driven by $\pi^M$. Then from $\pi(x) = \Khat x$ and $\pi^M(x) \in \left\{ \Khat x, 0 \right\}$, we have
\begin{align*}
    J & = \lim_{T\to\infty} \E \left[ \frac1T \sum_{k=0}^{T-1} \xhat_k^\top \left( Q + K^\top RK\right) \xhat_k \right] = \E \left[ \xhat^\top \left( Q + K^\top RK\right) \xhat \right] \\
    J^M & \leq \lim_{T\to\infty} \E \left[ \frac1T \sum_{k=0}^{T-1} x_k^\top \left( Q + K^\top RK\right) x_k \right] = \E \left[ x^\top \left( Q + K^\top RK\right) x \right],
\end{align*}
where $\xhat_k \xrightarrow{d} \xhat, x_k \xrightarrow{d} x$.
% TODO: prove existence of limiting/stationary distribution; prove temporal average = spacial average over stationary distribution
Therefore, we have
\begin{align*}
    J^M - J \sim \O \left( \E \norm{x}^2 - \E \norm{\xhat}^2 \right).
\end{align*}
To bound $\E \norm{x}^2 - \E \norm{\xhat}^2$, notice that
\begin{align*}
    x_k &= \left(A+B\Khat\right) x_{k-1}+w_{k-1} - B\Khat x_{k-1} \ind{u_{k-1} = 0} \\
    &= \left(A+B\Khat\right) \left( \left(A+B\Khat\right) x_{k-2}+w_{k-2} - B\Khat x_{k-2} \ind{u_{k-2} = 0} \right) +w_{k-1} - B\Khat x_{k-1} \ind{u_{k-1} = 0} \\
    &= \cdots \\
    &= \left(A+B\Khat\right)^k x_0 + \sum_{s=0}^{k-1} \left(A+B\Khat\right)^s w_{k-s-1} - \sum_{s=0}^{k-1}\left(A+B\Khat\right)^s B\Khat x_{k-s-1}\ind{u_{k-s-1} = 0} \\
    &= \xhat_k - \sum_{s=0}^{k-1}\left(A+B\Khat\right)^s B\Khat x_{k-s-1}\ind{u_{k-s-1} = 0}.
\end{align*}
From the fact that $\E(X_1+\cdots+X_n)^2 = \sum\limits_{i,j=1,\ldots,n} \E X_iX_j \leq \sum\limits_{i,j=1,\ldots,n} \sqrt{\E X_i^2\E X_j^2} = \left(\sqrt{\E X_1^2} + \cdots + \sqrt{\E X_n^2}\right)^2$, where $X_1,\ldots,X_n$ are possibly dependent random variables, it follows that
\begin{align*}
    \E \norm{x_k}^2
    &\leq \left( \sqrt{\E \norm{\xhat_k}^2} + \sum_{s=0}^{k-1} \norm{\left(A+B\Khat\right)^s B\Khat} \sqrt{\E\left[  \norm{x_{k-s-1}}^2 \ind{u_{k-s-1} = 0} \right]}\right)^2 \\
    &\leq \left( \sqrt{\E \norm{\xhat_k}^2} + \sum_{s=0}^{k-1} \norm{\left(A+B\Khat\right)^s B\Khat} \sqrt{\sqrt{\E  \norm{x_{k-s-1}}^4 } P(u_{k-s-1} = 0) }\right)^2 \\
    &\sim \left( \sqrt{\E \norm{\xhat_k}^2} + \O(1) \cdot \sum_{s=0}^{k-1} \norm{\left(A+B\Khat\right)^s }  P(u_{k-s-1} = 0) \right)^2 \\
    &\leq \left( \sqrt{\E \norm{\xhat_k}^2} + \O(1) \cdot \sum_{s=0}^{k-1}\sum_{\tau=0}^{t-1} \norm{\left(A+B\Khat\right)^s }  P\left( \norm{x_{k-s-\tau-1}} \geq M \right) \right)^2 \\
    &\sim \left( \sqrt{\E \norm{\xhat_k}^2} + \O(t) \cdot \sum_{s=0}^{k-1} \norm{\left(A+B\Khat\right)^s }  \O\left(1/M^2\right) \right)^2 \\
    &\sim \left( \sqrt{\E \norm{\xhat_k}^2} + \O\left(\frac{t}{M^2}\right)\right)^2,
\end{align*}
where in the third line we used $\E\norm{x_k}^4\sim \O(1)$ proved in our second step, in the fourth line we used the fact $\{u_{k} = 0\} \subset \cup_{\tau=0}^{t-1} \left\{ \norm{x_{k-t}} \geq M \right\}$ which is guaranteed by the update rule of $\safesteps$, in the fifth line we used $P\left(\norm{x_k} \geq M \right)\sim \O\left(\rho^k/M^2\right) \sim \O\left(1/M^2\right)$ proved in our first step, and in the sixth line we used the stability of $A+B\Khat$. Therefore, we have
\begin{align*}
    \E \norm{x_k}^2 - \E \norm{\xhat_k}^2 \sim O\left(\frac{t}{M^2}\right),
\end{align*}
which, according to our previous discussion, implies
\begin{align*}
    J^M - J \sim O\left(\frac{t}{M^2}\right).
\end{align*}
\end{proof}
